A Minimax Learning Approach to Off-Policy Evaluation in Confounded Partially Observable Markov Decision Processes

We consider off-policy evaluation (OPE) in Partially Observable Markov Decision Processes (POMDPs), where the evaluation policy depends only on observable variables and the behavior policy depends on unobservable latent variables. Existing works either assume no unmeasured confounders, or focus on settings where both the observation and the state spaces are tabular. In this work, we first propose novel identification methods for OPE in POMDPs with latent confounders, by introducing bridge functions that link the target policy's value and the observed data distribution. We next propose minimax estimation methods for learning these bridge functions, and construct three estimators based on these estimated bridge functions, corresponding to a value function-based estimator, a marginalized importance sampling estimator, and a doubly-robust estimator. Our proposal permits general function approximation and is thus applicable to settings with continuous or large observation/state spaces. The nonasymptotic and asymptotic properties of the proposed estimators are investigated in detail.

==> bandit.tex <==
\section{OPE in Partially Observable Contextual Bandits }\label{sec:bandit}

As a warm-up, we start with a partially observable contextual bandit setting (which is a special case of the above POMDP setting with horizon equals 1) to illustrate the challenge of OPE with latent confounders and present our main idea. Suppose we have $N$ data tuples that are i.i.d. copies of $\{O_{-1},A_0,O_0,R_0\}$ where $O_{-1}$ denotes the additional observation that is conditionally independent of $(A_0,O_0,R_0)$ given $S_0$. 
%problem and present the identification strategy. 
%Recall we observe $\{O^{-}_0,A_0,O_0,R_0\}$. 
The corresponding causal diagram is depicted in \pref{fig:POMDP_bandit} \footnote{This is formalized following \citep{bareinboim2020pearl}. }. 

Our objective is to evaluate the mean outcome under a given evaluation policy $\pi^e$ that maps the observation space to a probability distribution function on the action space. To discuss the challenge of OPE with unmeasured confounders, we further assume that $\pi^e$ is a deterministic policy such that $\pi^e(a|o)$ is binary-valued for any $a$ and $o$, and use $\pi^e(o)$ to denote the action that the agent selects after observing $o$. The target policy's value can be represented as $\EE [\EE \{R_0|O_0;do(A_0=\pi^e(O_0))\}]$ %\masa{is this $\EE \{R_0;  do(A_0=\pi^e(O_0)) \}=\EE \{\EE\{R_0\mid O_0;  do(A_0=\pi^e(O_0)) \};  do(A_0=\pi^e(O_0)) \}=\EE [\EE\{R_0\mid O_0;  do(A_0=\pi^e(O_0)) \}]$ ?  I think the above notation is confusing. } 
where the first expectation is taken with respect to the marginal distribution of $O_0$ and $do$ denotes the do-operator \citep[see e.g.,][]{tian2012identifying}. %\masa{i changed the citation since do operator for the dynamic treatment is in tian's paper.} 
The notation $do(A_0 = \pi^e(O_0))$ means that the action $A_0$ is set to the value $\pi^e(O_0)$ irrespective of the value
of the latent state $S_0$. In other words, whatever relationship exists between $S_0$ and $O_0$, that relationship is no longer in effect when we adopt the policy $\pi^e$. When $S_0$ confounds the action-reward association, the conditional expectation $\EE \{R_0|O_0;do(A_0=\pi^e(O_0))\}$ %\masa{I think this one is better $\EE[R_0|O_0;do(A_0=\pi^e(O_0))]$} 
is in general not equal to $\EE (R_0|A_0=\pi^e(O_0),O_0)$. This is because the distribution under $do(A_0 = \pi^e(O_0))$ is different from that under
$A_0 = \pi^e(O_0)$. The former corresponds to the distribution depicted in \pref{fig:POMDP_bandit} without the pathway $S_0\to A_0$ colored in blue whereas the latter is the distribution with the pathway $O_0\to A_0$ removed. As such, directly applying classical methods that assume no unmeasured confounders would yield a biased value estimator. 
%We next introduce the do-operator $do$ to represent a (hard) intervention \citep[see e.g.,][]{pearl2009causality}. 
%\footnote{It has also a causal interpretation by using causal DAGs \cite{bareinboim2020pearl,richardson2017nested}. }.

If we were to observe $S_0$, following the standard OPE methods, we could identify the policy value using the IS or value function-based estimator, given by $$\EE\bracks{\eta_0(S_0,A_0)R_0}\quad \mathrm{or}\quad \EE\left[v_0(S_0)\right]\quad \mathrm{where}\quad v_0(S_0)\coloneqq q_0(S_0,\pi^e_0)=\sum_a q_0(s_0,a)\pi^e_0(a\mid S_0),$$
and $q_0(S_0,A_0)=\E[R_0\mid S_0,A_0]$, $\eta_0=\pi^e_0/\pi^b_0$ denotes the IS ratio.  However, since we cannot observe $S_0$, these methods are not applicable. 

%Being inspired by \cite{cui2020semiparametric,kallus2021causal}, as a first step, we introduce bridge functions and assume the existence:  
To handle unmeasured confounders, we first assume the existence of certain bridge functions that link the target policy's value and the observed data distribution. %Similar ideas were proposed by \cite{cui2020semiparametric,kallus2021causal} under a different model setup. 
\begin{assum}[Existence of bridge functions]\label{assum:key}
There exist functions $b'_V:\Acal\times \Ocal \to \RR,b'_W:\Acal\times \Ocal\to \RR$ that satisfy $\forall (a,s)\in \{(a,s)\in \Acal\times \Scal:\E[\epol(a\mid O_0)\mid S=s]>0\}$: 
\begin{align}\label{eq:bridge}
   \EE[b'_V(A_0,O_0)\mid S_0=s,A_0=a] &= \EE[R_0 \pi^e(A_0 \mid O_0)\mid A_0=a,S_0=s],\\
    \E[b'_W(A_0,O_{-1})\mid S_0=s,A_0=a] &=1/\pi^b(a\mid s). \label{eq:bridge2}
\end{align}
We refer to $b'_V(\cdot)$ as value bridge functions and $b'_W(\cdot)$ as weight bridge functions. 
\end{assum}

By definition, weight bridge and value bridge functions can be interpreted as projections of the importance sampling weight (i.e., inverse propensity score) and value functions defined on the latent state space onto the observation space. 
%Weight bridge functions serve as importance weights (a.k.a., inverse propensity scores) $1/\pi^b$ and reward bridge functions serve as state-value functions.  
When  $\Scal$ and $\Ocal$ are discrete, the existence of solutions to the integral equations in \pref{eq:bridge} and \pref{eq:bridge2} %reduces to the non-singularity of some matrices as we will see in 
are equivalent to certain matrix rank assumptions. See
Assumption \ref{asm:weak1} introduced later for details. When $\Scal$ and $\Ocal$ are continuous, it follows from Picard's theorem \cite[Theorem 2.41]{carrasco2007linear} that Assumption \pref{assum:key} %the existence further 
 is implied by certain completeness conditions. Finally, it is worthwhile to mention that we do \emph{not} require these bridge functions to be uniquely defined. %{\color{blue} 
% In contrast, some existing works in the causal inference literature impose such uniqueness assumptions \citep{miao2018identifying,cui2020semiparametric}. 
 %which can be violated in settings .


Next, we show that Assumption \pref{assum:key} is a sufficient condition for policy value identification. Our identification method is more general than \cite{nair2021spectral,tennenholtz2020off} since their results are restricted to the tabular setting.  The following theorem shows that if we know $b'_V$ and $b'_W$ in advance, we can consistently estimated the target value $J(\pi^e)$ from the offline data. 

\begin{lemma}[Pseudo identification formula]\label{lem:first_step}
Suppose Assumption \ref{assum:key} holds. Then, for any $b'_V,b'_W $ that solve \pref{eq:bridge}, we have 
\begin{align}\label{eq:key}
    J(\pi^e)=\EE\bracks{\sum_a b'_V(a,O_0)}\quad\hbox{and}\quad J(\pi^e)=\EE[b'_W(A_0,O_{-1})R_0\pi^e(A_0\mid O_0)]. 
\end{align}
\end{lemma}
%The formula is the counterpart of IS formula. The second formula is the counterpart of the value function based formula. 
These formulas outline an IS estimator and a value function-based estimator for $J(\pi^e)$. It remains to identify the bridge functions $b_V'$ and $b_W'$. However, even if Assumption \ref{assum:key} holds, it is still very challenging to learn $b_V'$ and $b_W'$ from the observed data as their definitions involve the unobserved state $S_0$. As such, we refer to \pref{lem:first_step} as the ``pseudo" identification formula. In the following, we introduce some versions of bridge functions that are identifiable from the observed data. 
%since the definition of bridge functions involves the unobserved random variable $S_0$, we cannot identify $b_V$ and $b_W$ from the observed data. Nevertheless, we can identify similar functions defined as follows. 

\begin{definition}[Learnable bridge functions]\label{def:observed_bridge_bandit}
The learnable value bridge function $b_V:\Acal\times \Ocal \to \RR$ and weight bridge function $b_W:\Acal\times \Ocal \to \RR$ are solutions to 
\begin{align}\label{eq:observed}
\begin{split}
   \E[R_0\epol(A_0\mid O_0)\mid A_0,O_{-1}] &=\E[b_V(A_0,O_0)\mid  A_0,O_{-1}]\quad\hbox{and}\\ 
   1/P_{\bpol}(A_0\mid O_0) &=  \E[b_W(A_0,O_{-1}) \mid A_0,O_0 ], 
   %& \E[f(O_0,a)-b'_W(A_0,O_0)\mathbb{I}(A_0=a)f(O_0,A_0)]=0 .
\end{split} 
\end{align}
respectively. 
\end{definition}
Throughout this paper, we use $b'$ to denote the bridge function and $b$ to denote the learnable bridge function.


%Notably, bridge functions are observed bridge functions. 
The following lemma shows that any bridge function is a learnable bridge function. 
\begin{lemma}\label{lem:observed}
Bridge functions defined as solutions to \pref{eq:bridge} and  \pref{eq:bridge2} are learnable bridge functions. 
\end{lemma}
%We  remark $b_W$ is equivalently defined in the following way. 
We next present an equivalent definition for $b_W$.
This characterization is useful when extending our results to the POMDP setting. 
\begin{lemma}\label{lem:some_characterization}
$\E[b_W(A_0,O_{-1})\mid A_0,O_0]=1/\pi^b(A_0\mid O_0)$ holds if and only if $$\E[\sum_a f(O_0,a)-b_W(A_0,O_{-1})f(O_0,A_0)]=0,\quad \forall f:\Ocal\times \Acal \to \RR$$
\end{lemma}
%Still, the results so far are not enough for the identification since observed bridge functions are \emph{not} necessarily bridge functions; thus, we cannot invoke \pref{lem:first_step}. The following theorem shows that we can surprisingly plug observed bridge functions into \pref{eq:key} under Assumption \ref{assum:key}. 
As we have commented, the class of bridge functions are difficult to estimate from the observed data. On the other hand, the class of learnable bridge functions is identifiable. However, they are \emph{not} necessarily bridge functions. Thus, we cannot invoke \pref{lem:first_step} for value identification. Nonetheless, perhaps surprisingly, the following theorem shows that we can plug-in any learnable bridge function $b_V$ and $b_W$ for $b_V'$ and $b_W'$ in \pref{eq:key} under Assumption \ref{assum:key}. 

%\masa{I also changed. }
\begin{theorem}[Key identification formula]\label{thm:final_step}
\begin{enumerate}~
    \item Assume the existence of value bridge functions and learnable weight bridge functions. Then, letting $b_W(\cdot)$ be a learnable weight bridge function, 
    \begin{align*}
    J(\epol)=\E[b_W(A_0,O_{-1})R_0] . 
\end{align*}
\item Suppose the existence of weight bridge functions and learnable value bridge functions. Then, letting $b_V(\cdot)$ be a lernable value bridge function, 
\begin{align*}
 J(\epol)=\E[\sum_a b_V(a,O_0) ] . 
\end{align*}
\end{enumerate}
\end{theorem}

%\masa{i edit this paragraph}
We make a few remarks. First, the assumptions in the first and second statements do not imply each other. In both cases, Assumption \ref{assum:key}, the existence of bridge functions, plays a critical role in ensuring the validity of the above equations. Specifically, when Assumption \ref{assum:key} holds, the assumptions in both the first and second statements are automatically satisfied, since bridge functions are learnable bridge functions.
%Assumption \ref{assum:key} implies the first and second assumption recalling bridge functions are learnble bridge functions. 
%\begin{remark}
%Assumption \pref{assum:key} plays a critical role in ensuring the validity of the above equations, 
%stress out that Assumption \pref{assum:key} still plays the critical role 
%although $b_V$ and $b_W$ are not necessarily bridge functions.
%Assumption \pref{assum:key}  ensures the existence of observed bridge functions satisfying \pref{eq:observed}.
If we naively replace Assumption \ref{assum:key} with the existence of learnable bridge functions that satisfy \eqref{lem:observed}, then \pref{thm:final_step} is no longer valid. 

Second, Theorem \ref{thm:final_step} implies that we only need bridge functions to exist, but do not need to identify them. As long as they exist, learnable bridge functions can be used for estimation, which are not necessarily bridge functions. 
%\end{remark}
%Some readers might wonder whether Assumption \ref{assum:key} is replaced with the existence of observed bridge functions since at a first glance, the observed bridge functions appear in the formulas but not bridge functions themselves. However, then the theorem breaks down. 
%\begin{remark} \


Third, similar identification methods have been developed in the causal inference literature for evaluating the average treatment effect with double negative controls \citep{kallus2021causal} based on \cite{miao2018identifying,cui2020semiparametric}. However, their settings differ from ours. 
%For instance, all the aforementioned works consider state-agnostic evaluation policies, i.e., policies that are constant functions of observations. 
For instance, all the aforementioned works consider negative-control-agnostic evaluation policies, i.e., policies that are constant functions of negative controls. In contrast, we allow our evaluation policy to depend on the observation which serves as negative controls in their setting.
%(i.e., $O_0$).  \masa{Here, since the other works's (\citep{kallus2021causal}) evaluation polices can depend on the observations, which are not used as negative controls, i changed the expression. }
%In addition, {\color{blue}they require the bridge functions to be uniquely defined}. 
%\end{remark}
%suppose that evaluation policies do not depend on $O_0$. 

\begin{comment}
\begin{remark}[Difference comparing to standard negative controls literature] 
The closely related identification strategy has been extensively studied in the causal inference literature with unmeasured confounders \cite{miao2018identifying,kallus2021causal,cui2020semiparametric}. As the most closely related work, we take an approach in \cite{kallus2021causal}. If we take another approach \cite{cui2020semiparametric}, we need additional assumptions such as the strong completeness assumption \footnote{This assumption has nothing to do with the so-called Bellman completeness in the RL setting \cite{chen2019information}. }. While the standard contextual bandit setting and the standard causal inference setting with no unmeasured confounders are essentially equivalent, the POMDP setting we consider differs from the settings in the above-mentioned literature. All of these works suppose that evaluation policies do not depend on $O_0$.  
\end{remark}
\end{comment}

To conclude this section, we specialize our results to the discrete setting where $\Scal,\Ocal$ and the reward space are all discrete. In that case, 
%\paragraph{Discrete setting} \label{rem:discrte}
%When $\Scal,\Ocal$ and reward space are discrete,  
since integral equations can be represented in matrix form, Assumption \ref{assum:key} is immediately implied by the following conditions. 
\begin{assum}\label{asm:weak1}
$\rank(\Prr_{\bpol}(\bO_0\mid \bS_0))= |\Scal|$ and $\rank(\Prr_{\bpol}(\bO_{-1}\mid \bS_0))= |\Scal|$. 
\end{assum}
This assumption essentially requires that the state space is sufficiently informative. It implies that $|\Ocal|\geq |\Scal|$. Such an assumption is weaker than the one imposed in \cite{tennenholtz2020off} that requires the state and observation spaces have the same cardinality. The following lemma states that Assumption \pref{asm:weak1} is equivalent to Assumption 2 in \cite{nair2021spectral}.

\begin{lemma}\label{lem:equivalence}
Assumption \pref{asm:weak1} holds if and only if 
$\rank(\Prr_{\bpol}(\bO_0 \mid A_0=a,\bO_{-1}))= |\Scal|,\forall a\in \Acal$, which is an assumption in  \cite{nair2021spectral}. 
\end{lemma}
Then, following \cite{nair2021spectral}, the policy value can be explicitly identified as follows: 
\begin{theorem}[Identification formula in the tabular setting]\label{thm:discrete_identify}
\begin{align*}
    J(\pi^e)=\sum_{a,r,o}r\pi^e(a\mid o)\Prr_{\bpol}(r,o\mid \bO_{-1})\{\Prr_{\bpol}(\bO_0\mid A_0=a,\bO_{-1})\}^{+}\Prr_{\bpol}(\bO_0). 
\end{align*}
\end{theorem}




\begin{figure}[!t]
\centering
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=0.8\linewidth]{main_document/bandit_graph.pdf}
  \caption{Partially Observable Contextual Bandits}
  \label{fig:POMDP_bandit}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=\linewidth]{main_document/POMDP_graph.pdf}
  \caption{Time-homogeneous POMDPs.} %{\color{blue} \{CS: Masa, would you please change this figure by introducing $S^-$ and $A^-$? In addition, there shall be an edge from $A$ to $S^+$.\} }}
  \label{fig:POMDP_homo}
\end{subfigure}
\caption{Red lines depict the dependency of evaluation policies on the observed variables. Blue lines depict the dependence of behavior policies on the state variables. }
%\label{fig:test}
\end{figure}

==> experiment.tex <==
\section{Experiments}
\subsection{Experiments on Toy Example with Linear Function Approximator}
We choose $\gamma = 0.95$ in all the experiments in this section. Besides, for simplicity, we will alternatively use PO-MQL are PO-MWL to refer to the method based on solving value bridge functions $b_v$ and weight bridge functions $b_w$, respectively, and use PO-DR to refer to their doubly-robust version.
\paragraph{Measure of Estimation Error}
Given $n$ dataset $D_1,D_2,...,D_n$, the estimators computed based on each dataset $\hat{V}_1,...,\hat{V}_n$, and the true value $V$, we define the relative bias to be:
\begin{align*}
    |\frac{1}{n}\sum_{i=1}^n \frac{\hat{V}_i}{V}-1|.
\end{align*}
and define the relative Mean-Squared Error (MSE) to be:
\begin{align*}
    |\frac{1}{n}\sum_{i=1}^n\Big(\frac{\hat{V}_i-V}{V}\Big)^2|.
\end{align*}
In our experiments, we mainly use the above two methods as the measure of estimation error of estimators.
\subsubsection{Setting}
\paragraph{Environment}
We consider a one-dimensional continuous dynamic process as a toy example, and the initial distribution, the transition and reward function are defined by:
\begin{align*}
    S_0\sim \mathcal{N}(0,0.5^2),\quad S_{t+1} = \frac{1}{2} S_t + \delta \cdot (2A_t - 1) + \mathcal{N}(0, \sigma_S^2),\quad R_{t+1} = S_{t+1} + \delta \cdot (2A_t-1).
\end{align*}
where $\delta$ is a weighted factor and $\sigma_S$ reflects the randomness of the transition. In the following experiments, we fix $\delta=1.0$, and $\sigma_S = 0.5$. 
Besides, the observation is computed by adding noise on the state:
\begin{align*}
    O_t \gets S_t + \mathcal{N}(0,\sigma_O^2)
\end{align*}
\paragraph{Choice of Behavior and Target Policies}
We consider the Sigmoid policy to be behavior and target policies, i.e.:
\begin{align*}
    \pi^S_{w}(\cdot|S) \sim \frac{1}{1+\exp(-wS+1)},\quad \pi^O_{w}(\cdot|O) \sim \frac{1}{1+\exp(-wO+1)}
\end{align*}
We use $\pi_{-1}^S$ (i.e. $w=-1$) as the behavior policy to generate the data. The dataset $D$ consists of trajectories starting from initial state with horizon length equal 100. As for the target policies, we choose multiple different $w$ around $w=-1$, including $\pi^O_{-3},\pi^O_{-2},\pi^O_{1},\pi^O_{2}$.

\paragraph{Evaluating Process}
We evaluate the linear estimator discussed in Example \ref{example:linear_model} (Note that the MWL, MQL and DR collapse to the same linear estimator, and so do PO-MWL, PO-MQL, PO-DR). In order to reduce the approximation error of linear function class,  approximation error of linear function class, we use $\mathcal{V}:= \{(a,o) \rightarrow \pi^e(a|o)\theta^\top\phi(a,o):\theta \in \Theta\}$ instead, since $b_v$ is expected to approximate the product between $\pi^e(a|o)$ and some value function. As a result, the new linear estimator of our method would be:
\begin{align*}
	\E_{O\sim\nu_O,a\sim \pi^e(\cdot|O)}[\phi(a,O)]^{\top}\big(\E_{\Dcal}[&\phi(A,O^{-})\phi^{\top}(A,O)\epol(A\mid O) \\
	&-\gamma  {\phi(A,O^{-})\epol(A\mid O) \EE_{a'\sim\epol(\cdot|O^+)}[\phi^{\top}(a',O^+)]}]\big)^{+}\E_{\Dcal}[R \epol(A\mid O)\phi(A,O^-)].
\end{align*}
Since the baseline method do not need to use the same trick, the linear estimator for baseline method is the same one as mentioned in Example \ref{example:linear_model}:
\begin{align*}
	\E_{\Dcal}[\phi(\epol,S)]^{\top}\prns{\E_{\Dcal}[\phi(A,S)\phi^{\top}(A,S)] -\gamma  \E_{\Dcal}\bracks{\phi(A,S)\phi^{\top}(\epol,S^+)} }^{+}\E_{\Dcal}[R \phi(A,S)], 
\end{align*}
where $\phi(\epol,s)=\E_{a\sim \epol(s)}[\phi(a,s)]$. 

As for the choice of linear feature, we use the sklearn.kernel\_approximation.RBFSampler (\url{https://scikit-learn.org/stable/modules/generated/sklearn.kernel_approximation.RBFSampler.html}) to generate the linear features. We choose the RBF kernel to be $\exp(-5\cdot x^2)$, and the feature dimension is 100.

\subsubsection{Experiment Results}
We generate 10 datasets with the behavior policy and 10 different random seeds. For each dataset, and each target policy, we use 5 different random seeds to generate the 5 different sets of RBF features, and report the average of the estimation with them as the estimation result of the target policy given the dataset. 

\paragraph{Comparison under Different Noise Level}
In the first experiment, we evaluate the results when $\sigma_O = 0.5,1.0,1.5$. The sample size of the dataset $D$ size is $|D| = 200000$, which corresponds to 2000 trajectories $N_D=2000$. 

For each noise level and each target policy, we compute (the log level) relative bias and the relative MSE (with error bar corresponding to double standard error, i.e. 96\% confidence interval) for both ours and baseline methods, and report the results in Figure \ref{fig:Toy_Varying_NoiseLevel0.5}, \ref{fig:Toy_Varying_NoiseLevel1.0} and \ref{fig:Toy_Varying_NoiseLevel1.5}. As we can see that, when the noise size $\sigma_O$ is small, our method is comparable with the baseline. Moreover, as the increase of $\sigma_O$, the baseline method will suffer from much higher bias than ours.
\begin{figure}[H]
    \centering
    \includegraphics[scale=0.35]{ExpFigures/Toy_N0.5_Bias.png}
    \includegraphics[scale=0.35]{ExpFigures/Toy_N0.5_MSE.png}
    \caption{$\sigma_O = 0.5$. Left: Log of bias; Right: Log-MSE}
    \label{fig:Toy_Varying_NoiseLevel0.5}
\end{figure}
\begin{figure}[H]
    \centering
    \includegraphics[scale=0.35]{ExpFigures/Toy_N1.0_Bias.png}
    \includegraphics[scale=0.35]{ExpFigures/Toy_N1.0_MSE.png}
    \caption{$\sigma_O = 1.0$. Left: Log of bias; Right: Log-MSE}
    \label{fig:Toy_Varying_NoiseLevel1.0}
\end{figure}
\begin{figure}[H]
    \centering
    \includegraphics[scale=0.35]{ExpFigures/Toy_N1.5_Bias.png}
    \includegraphics[scale=0.35]{ExpFigures/Toy_N1.5_MSE.png}
    \caption{$\sigma_O = 1.5$. Left: Log of bias; Right: Log-MSE}
    \label{fig:Toy_Varying_NoiseLevel1.5}
\end{figure}

\subsubsection{Comparison under Different Sample Size}
In this experiment, we report the results when the number of samples in the dataset is at different level, including $|D|=$5e4, 1e5 and 2e5. The results are plotted in Figure \ref{fig:Toy_Varying_SampleSize}.

As we can see, when gradually increasing the sample size, the estimation error of our methods gradually decrease and become smaller than baseline estimators, because the variance/noise of the estimation decays as the sample size increasing and our methods have much smaller bias.
In contrast, the estimation error of the baseline estimator stay high and almost does not change even if the dataset becomes larger, which indicates that the main origin of the estimation error of baseline method is its inherent bias.
% \begin{figure}[H]
%     \centering
%     \includegraphics[scale=0.5]{ExpFigures/Toy_SampleSize_Bias.png}
%     \includegraphics[scale=0.5]{ExpFigures/Toy_SampleSize_MSE.png}
%     \caption{Experiments with varying sample size. Noise Level $\sigma_O=1.0$}
%     \label{fig:Toy_Varying_SampleSize}
% \end{figure}
\begin{figure}[H]
    \centering
    \includegraphics[scale=0.4]{ExpFigures/Toy_VarySS_Bias.png}
    \includegraphics[scale=0.4]{ExpFigures/Toy_VarySS_MSE.png}
    \caption{Experiments with varying sample size. Noise Level $\sigma_O=1.0$}
    \label{fig:Toy_Varying_SampleSize}
\end{figure}

\subsection{Experiments on CartPole with Neural Network}
\subsubsection{Setting}
\paragraph{Environment}
The state space is 4D, including position and velocity of cart, and angle and angle velocity of pole. The action space is $\{0,1\}$, corresponding to move towards left/right. Besides, we use a revised reward function which allows the value of different policies are more distinguishable and is defined below, instead of the simple indicator function depending on whether the pole is fallen:
\begin{align*}
    r = |2.0 - \frac{x}{x_{\text{clip}}}|\cdot |2.0 - \frac{\theta}{\theta_{\text{clip}}}| - 1.0
\end{align*}
where $x$ and $\theta$ are the position of Cart and angle of Pole, respectively, and $x_{\text{clip}}$ and $\theta_{\text{clip}}$ are the threshold that the episode will terminate (done = True) as long as either $|x| \geq x_{clip}$ or $|\theta| \geq \theta_{clip}$. The reward will be higher when the Cart is closer to the center and the angle of Pole is closer to perpendicular. It's easy to observe that $r\in[0,3]$ so that the value range is $[V_{\min}, V_{\max}]$ with $V_{\min}=0$ and $V_{\max}=60$ when $\gamma=0.95$.

Besides, the observation is created by adding relative noise on states in the following way:
\begin{align*}
    O = S * (1+ \epsilon),\quad \epsilon \sim \mathcal{N}(0, \sigma) \in \mathbb{R}^4
\end{align*}
where * is the element-wise multiplication operator.
Here, we use the $S(1+ \epsilon)$ instead of $S + \epsilon$ because value range of the each state dimension are different. We fix the $\sigma=0.1$ in all the experiments in this section.
\paragraph{Choice of Behavior and Target Policies}
For the behavior policy, we first use DQN to train a near-optimal policy $\pi^*_S$, and convert the well-trained Q function $Q_S$ to a softmax policy in the following way:
\begin{align*}
    \pi_S(\cdot|S) \propto \exp(-\frac{Q_S(S,\cdot)}{\tau_S}).
\end{align*}
and we fix $\tau_S=5.0$ in the following experiments.

As for the target policy, similarly, we train a Q network $Q_O$ with DQN on PO-MDP to obtain a near-optimal policy, and convert it to a softmax policy:
\begin{align*}
    \pi_O(\cdot|O) \propto \exp(-\frac{Q_O(O,\cdot)}{\tau_O}).
\end{align*}
for some temperature $\tau_O$.
\subsubsection{Function Approximator and Loss Function}
We follow the \citep{uehara2020minimax} and use the kernel function class. Both $b_v$ in PO-MQL and $b_w$ in PO-MWL are parameterized by a two-layer neural network with layer width = 256 and ReLU as activation function, and are optimized by kernel loss function (as we will introduce the derivation below), which corresponds to the case when adversarial function belongs to some particular kernel function class.

In the following, we will use $K(x_1;x_2)$ to denote the RBF kernel:
\begin{align*}
    K(x_1;x_2) := \exp(-\frac{\|x_1-x_2\|_2}{2\beta^2})
\end{align*}
where $\beta$ is the bandwidth. We choose $\beta = \text{med}/2$ during the training of PO-MWL ($b_w$) or MWL, and $\beta = \text{med}/5$ for PO-MQL ($b_v$) or MQL, where ``med'' is the median of the l2-distance over the samples in the dataset.
\paragraph{Derivation of the Loss Function for PO-MQL ($b_v$)}
Similar to the experiments in Toy environments, we reparameterize $g$ function with $\bar{g}\cdot \pi^e$, and therefore the predictor with $g$ should be adjusted by replacing $g$ with $\bar{g}\cdot \pi^e$:
\begin{align*}
    \EE_{O\sim \nu_O,A\sim \pi^e}[\bar{g}(O,A)\pi^e(A|O)].
\end{align*}
and the loss function is derived by:
\begin{align*}
    \max_f L_V^2(g,f)  =& \max_f \Big(\E[(R\pi^e(A|O)+\gamma \E_{a'\sim\pi^e}[g(a',O^+)]\pi^e(A|O)-g(A, O)\pi^e(A|O))f(A,O^-)]\Big)^2\\
    =&\max_f \Big(\Big\langle f, \E[R\pi^e(A|O)+\gamma \E_{a'\sim\pi^e}[g(a',O^+)]\pi^e(A|O)-g(A, O)\pi^e(A|O)]K(A,O^-;\cdot)\Big\rangle_{\mathcal{H}_K}\Big)^2\\
    =&\E[\Big(R\pi^e(A|O)+\gamma \E_{a'\sim\pi^e}[g(a',O^+)]\pi^e(A|O)-\pi^e(A|O)g(A, O)\Big)K(A,O^-;\barA,\barO^-)\\
    &\cdot\Big(\bar{R}\pi^e(\barA|\barO)+\gamma \E_{\bar{a}'\sim\pi^e}[g(\bar{a}',\barO^+)]\pi^e(\barA|\barO)-\pi^e(\barA|\barO)g(\barA,\barO)\Big)].\label{eq:kernel_loss_of_bv}
\end{align*}
\paragraph{Derivation of the Loss Function for PO-MWL ($b_w$)}
Similarly, we reparameterize $f$ function with $\bar{f}\cdot \pi^e$. Since we do not change the parameterization of $b_w$, we only need to adjust the loss function without changing the estimator:
\begin{align*}
    &\max_f L^2_W(g,f) \\
    =&\max_f \Big(\E[\gamma g(O^-,A)\pi^e(A|O)\sum_{a'}f(O^+,a')-g(O^-,A)f(O,A)]+(1-\gamma)\E_{O\sim \nu_O}[\sum_{a'}f(O,a')]\Big)^2\\
    =&\max_f \Big(\E[\gamma g(O^-,A)\pi^e(A|O)\E_{a'\sim \pi^e(\cdot|O^+)}[\bar{f}(O^+,a')]-g(O^-,A)\pi^e(A|O)\bar{f}(O,A)]+(1-\gamma)\E_{O\sim \nu_O,a'\sim\pi^e}[\bar{f}(O,a')]\Big)^2\\
    =&\max_f \Big(\E[\gamma g(O^-,A)\pi^e(A|O)\E_{a'\sim \pi^e(\cdot|O^+)}[\la \bar{f}, K(O^+,a'; \cdot)\ra]-g(O^-,A)\pi^e(A|O)\la \bar{f}, K(O,A;\cdot)\ra]\\
    &+(1-\gamma)\E_{O\sim \nu_O,a'\sim\pi^e}[\la \bar{f}, K(O,a';\cdot)\ra]\Big)^2\\
    =&\max_f \Big(\la \bar{f}, \E[\gamma g(O^-,A)\pi^e(A|O)\Big(\E_{a'\sim \pi^e(\cdot|O^+)}[K(O^+,a'; \cdot)]- K(O,A;\cdot)\Big)]+(1-\gamma)\E_{O\sim \nu_O,a'\sim\pi^e}[K(O,a';\cdot)]\ra\Big)^2\\
    =& \E[g(O^-,A)\pi^e(A|O)g(\barO^-,\barA)\pi^e(\barA|\barO)\cdot \\
    &\quad\quad\quad\Big(\gamma^2 K(O^+,\pi^e;\barO^+,\pi^e)+ K(O,A;\barO,\barA)-\gamma K(O^+,\pi^e;\barO,\barA)-\gamma K(O,A;\barO^+,\pi^e)\Big)]\\
    &+(1-\gamma)^2\E[K(O_0,\pi^e;\barO_0,\pi^e)]\tag{no gradient}\\
    &+\gamma(1-\gamma) \E[g(O^-,A)\pi^e(A|O) K(O^+,\pi^e;\barO_0,\pi^e)+g(\barO^-,\barA)\pi^e(\barA|\barO) K(O_0,\pi^e;\barO^+,\pi^e)]\\
    &- (1-\gamma) \E[g(O^-,A)\pi^e(A|O)K(O,A;\barO_0,\pi^e)+g(\barO^-,\barA)\pi^e(\barA|\barO)K(O_0,\pi^e;\barO,\barA)].
\end{align*}
where we denote 
$$K(O,\pi^e;\barO, \pi^e):=\E_{a'\sim \pi^e(\cdot|O), \bar{a}'\sim \pi^e(\cdot|\barO)}[K(O,a';\barO, \barA),\quad K(O,\pi^e;\barO, \barA):=\E_{a'\sim \pi^e(\cdot|O)}[K(O,a';\barO, \barA)].$$


\paragraph{Loss Function of Baseline Estimators}
We follow the \citep{uehara2020minimax} about the derivation of MQL and MWL loss function with kernel function class setting. The loss function of MQL is defined by:
\begin{align*}
    \max_f L_q^2(f,q)=& \E[\Big(R+\gamma \E_{a'\sim\pi^e(\cdot|O^+)}[ q(a',O^+)]-q(A, O)\Big)K(A,O;\barA,\barO)\Big(\bar{R}+\gamma \E_{\bar{a}'\sim\pi^e(\cdot|\barO^+)}[ q(\bar{a}',\barO^+)]-q(\barA,\barO)\Big)].
\end{align*}
and the loss of MWL is:
\begin{align*}
    &\max_f L_w^2(f,w)\\
    =&\E[w(O,A)w(\barO,\barA)\Big(K(O^+,\pi^e;\barO^+,\pi^e)+ K(O,A;\barO,\barA)-\gamma K(O^+,\pi^e;\barO,\barA)-\gamma K(O,A;\barO^+,\pi^e)\Big)]\\
    &+(1-\gamma)^2\E[K(O_0,\pi^e;\barO_0,\pi^e)]\tag{no gradient}\\
    &+\gamma(1-\gamma)\E[w(O,A)K(O^+,\pi^e;\barO_0,\pi^e)+w(\barO,\barA)K(O_0,\pi^e;\barO^+,\pi^e)]\\
    &-(1-\gamma)\E[w(O,A)K(O,A;\barO_0,\pi^e)+w(\barO,\barA)K(O_0,\pi^e;\barO,\barA)].
\end{align*}
Besides, we use the same neural network architecture and the same choice of bandwidth during the training of MQL/MWL as those for PO-MDP.
\paragraph{Experiment Results}
We collect the dataset by using the behavior policy to sample trajectories until the sample size reaches 200000, and generate 10 dataset with 10 different random seeds. For each dataset, we train the NN by minimize the loss function introduced above with learning rate 5e-3 for 10000 iterations. We record the prediction error for every 100 iterations and use the average of the last 10 records as the final estimation results given that dataset (corresponding to the prediction at iterations from 9100 to 10000 with 100 as interval).

We use several different choice of $\tau_O$ around $\tau_S=5.0$ to compute the behavior policies. We report the relative bias and MSE in Figure \ref{fig:CartPole_Results}. As we can see, our methods (PO-MWL, PO-MQL and PO-DR) can achieve smaller estimation error than baseline methods (MWL, MQL and DR). As the increase of $\tau_O$, the softmax target policy will behave more similar to a uniform policy, which results in less confounding, and leads to the decrease of the advantage of our methods.
\begin{figure}[H]
    \centering
    \includegraphics[scale=0.5]{ExpFigures/CartPole_KernelFuncAppx_Bias.png}
    \includegraphics[scale=0.5]{ExpFigures/CartPole_KernelFuncAppx_MSE.png}
    \caption{Comparison of results on CartPole environment. We use red, blue, green to mark (PO-)MWL, (PO-)MQL, and (PO-)DR respectively, and use dashed lines and solid lines to distinguish ours and baseline methods.}
    \label{fig:CartPole_Results}
\end{figure}


==> preliminary.tex <==

\section{Problem Formulation}%Preliminary}

We consider a finite-horizon discounted Partially Observable Markov Decision Process (POMDP) %. A POMDP is 
defined as $\langle \Scal,\Acal,\Ocal, \{r_t\}_{t\ge 0},\{P_t\}_{t\ge 0},\{Z_t\}_{t\ge 0},\gamma \rangle$, where $\Scal$ denotes the state space, $\Acal$ denotes the finite action space, $\Ocal$ denotes the observation space, $P_t:\Scal \times \Acal \to \Delta(\Scal)$ denotes %a (possibly time-dependent) 
the state transition kernel at time $t$, $Z_t:\Scal\to \Delta(\Ocal)$ denotes the observation function that defines the conditional distribution of the observation given the state at time $t$, $r_t:\Scal\times \Acal \to [0,1]$ denotes the reward function that depends on the state-action-next state triplet at time $t$, and $\gamma\in [0,1)$ is a discount factor that balances the immediate and future rewards. %All of 
$P_t,r_t$ and $Z_t$ are unknown to us and need to be estimated from the observed data. 
%a priori. 

The data generating process in POMDPs is depicted in Figure \ref{fig:POMDP}. It can be formulated as follows. 
%In a POMDP, 
Suppose the environment is in a given state
%in a state 
$s\in \Scal$. The agent selects an action $a\in\Acal$. Then the system transits into a new state $s'$ and gives an immediate reward $r(s,a)$ to the agent.
%and receives a reward whose conditional expectation equals $r(s,a)$. 
While we cannot directly observe the latent state $s$, we have access to an observation $o\sim Z(\cdot|s)$. %Given a set of polices 
A policy is a set of time-dependent decision rules $\pi=\{\pi_t\}$ where each $\pi_t:\Scal\times \Ocal \to \Delta(\Acal)$ maps the state-observation pair to a probability distribution over the action space. For %a given 
%\masa{I removed a given since it is not in time inhomogeneous setting.}
%an initial state distribution $\nu_0\in \Delta(\Scal)$ and the 
a given policy $\pi$, %and POMDP together generates a trajectory of length $t$, i.e.,
the data trajectory up to time $t$ can be summarized as $O_{\cj_t}=(S_0,O_0,A_0,R_0,\cdots,S_t,O_t,A_t,R_t)$ where %following 
$S_0\sim \nu_0,O_0\sim Z_0(\cdot|S_0),A_0\sim \pi_0(\cdot|S_0),R_0=r_0(S_0,A_0),S_1\sim P_0(\cdot|S_0,A_0),\cdots$ where $\nu_0$ denotes the initial state distribution. %where each $\varepsilon_t$ is some mean-zero random error independent of the past data history. %An observable trajectory of length 
The observed data up to $t$ is %defined 
given by $\tau_t=(O_0,A_0,R_0,\cdots,O_t,A_t,R_t)$. We denote its distribution by $P_{\pi}$. The policy value $J(\pi)$ is defined as the expected cumulative reward $\E_{\pi}[\sum_{t=0}^{H}\gamma^t R_t]$ for some $0<H\le +\infty$, where the expectation is taken w.r.t.~the distribution of trajectories induced by  policy $\pi$. 
%under a policy $\pi$ and the above-mentioned POMDP.  

\begin{figure}[!t]
    \centering
  \includegraphics[width=\linewidth]{./main_document/POMDP.pdf}
    \caption{The data generating process in POMDPs. The evaluation policy in red depends on the observed variables. The behavior policy depends on the hidden state variables. }
    \label{fig:POMDP}
\end{figure}

%We study off-policy evaluation (OPE) in POMDPs following \cite{tennenholtz2020off}. In OPE, we consider two evaluation polices: an evaluation policy $\pi^e_t:\Ocal \to \Delta(\Acal)$ and a behavior policy $\pi^b_t:\Scal \to \Delta(\Acal)$ for $t=0,\cdots,H-1$. 
For a given evaluation policy $\pi^e=\{\pi^e_t\}_t$, %that depends on the state-observation pair only through the observation variable,
the goal of OPE is to evaluate $J(\pi^e)$ from an observational dataset that consists of $N$ data trajectories, %up to time $H$, 
generated by a behavior policy $\pi^b=\{\pi^b_t\}_t$. As shown in \pref{fig:POMDP}, we focus on the setting where $\bpol$ depends on the state-observation pair only through the state variables and $\epol$ depends on the observation variables only. %See Figure \pref{fig:POMDP} for a graphical illustration. 
%{\color{blue}\{CS: \it Would it be possible to relax this assumption?\}} \masa{looks no. i means $A\perp O\mid S$ looks critical.} 
Under this model assumption, the state variables serve as a confounder between the action and the reward at each time. Since the state is not fully observed, the no unmeasured confounder assumption is violated. 
%{\color{blue}We also assume the logged data includes an observation of some time step before the initial evaluation, and denote it by $O^{-}_0$.} 

To conclude this section, we introduce some notations. 
%We denote the observed $N$ trajectories by $\Dcal=\{\cj^{\langle i\rangle}\}_{i=1}^N$, and define $\EE_{\Dcal}[f]=1/N\sum_i f(\cj^{\langle i\rangle})$. 
The expectation $\EE[\cdot]$ without any subscript is taken with respect to the offline data generated by the behavior policy. The notation $X_n=o_p(a_n)$ means that $\lim_{n\to \infty} \P(|X_n/a_n|\geq \epsilon)=0$ for any $\epsilon>0.$
%the expectation regarding the logged data. 
%Throughout this paper, 
The state and observation spaces considered in this paper can be either discrete or continuous. When they are discrete, we use the following notation. Let $X,Y$ be random variables taking values $\{x_1,\cdots,x_n\}$ and $\{y_1,\cdots,y_m\}$, respectively. Then we denote a $n\times m$ matrix with elements $\mathrm{Pr}(x_i\mid y_j)$ by $\mathrm{Pr}(\mathbf{X}\mid \mathbf{Y})$. Similarly, $\Prr(\mathbf{X})$ denotes a $n$-dimensional vector with elements $x_i$. We denote the Moore-penrose inverse of $\mathrm{Pr}(\mathbf{X}\mid \mathbf{Y})$ by $\mathrm{Pr}(\mathbf{X}\mid \mathbf{Y})^+$. 
 

\input{main_document/bandit}


==> proof2.tex <==
\section{Omitted proof}


\subsection{Proof of \pref{sec:bandit} }


\begin{proof}[Proof of \pref{lem:first_step}]
First, we prove the value-function based identification formula: 
\begin{align*}
    &\E[\sum_{a}b'_{V}(a,O_0)]=\E[\sum_{a}\E[b'_{V}(a,O_0)|S_0]]=\E[\sum_{a}\E[b'_{V}(a,O_0)|A_0=a,S_0]]  \tag{$A_0\perp O_0 \mid  S_0 $}\\ 
    &=\E[\sum_{a}\E[R_0\pi^e(a|O_0)|A_0=a,S_0]]  \tag{Definition of bridge functions} \\ 
    &=\E[\sum_{a}\E[R_0|A_0=a,S_0]\E[\pi^e(a\mid O_0)\mid A_0=a,S_0]] \tag{$R_0 \perp O_0 \mid A_0,S_0$ }\\
    &=\E[\sum_{a}\E[R_0|A_0=a,S_0]\E[\pi^e(a\mid O_0)\mid S_0]]  \tag{$A_0 \perp O_0 \mid S_0$}\\
    &=\E[\sum_{a}\E[R_0|A_0=a,S_0]\pi^e(a\mid O_0) ]\\
    &=J(\epol).  \tag{From standard regression formula}
\end{align*}

Second, we prove the importance sampling identification formula: 
\begin{align*}
&\E[b_{W}(A_0,O^{-}_0)R_0\pi^e(A_0\mid O_0)] = \E[\E[b'_{W}(A_0,O^{-}_0) \mid S_0,A_0]R_0\pi^e(A_0\mid O_0)] \tag{$O^{-}_0 \perp R_0\mid S_0,A_0   $} \\
&= \E[1/\pi^b(A_0\mid S_0)\pi^e(A_0\mid O_0)R_0]\tag{Definition of $b'_W$ } \\
&=J(\epol).  \tag{From standard IPW formula}
    %&\E[\sum_{a}b_{W}(A,O^{-})R\pi^e(a\mid O)]=  \E[\sum_{a}\E[b_{W}(A,O^{-})\mid A,S,O,R]R\pi^e(a\mid O)] \\ 
    %&= \E[\sum_{a}\E[b_{W}(A,O^{-})\mid A,S]R\pi^e(a\mid O)]=\E\bracks{\sum_{a}\frac{\rI(A=a)}{b(a\mid O)} R\pi^e(a\mid O)}=\E\bracks{\frac{\pi^e(A\mid O)R}{\bpol(A\mid O) }} . 
\end{align*}
\end{proof}



\begin{proof}[Proof of \pref{lem:observed}]

We first prove reward bridge functions are learnable reward bridge functions: 
  \begin{align*}
     &\E[R_0\epol(A_0|O_0)\mid A_0,O^{-}_0]=\E[\E[R_0\epol(A_0|O_0)\mid A_0,S_0,O^{-}_0]\mid A_0, O^{-}_0]\\
     &=\E[\E[R_0\epol(A_0|O_0)\mid A_0,S_0]\mid A_0, O^{-}_0] \tag{$R_0, O_0 \perp O^{-}_0 \mid S_0,A_0 $ }\\ 
     & = \E[\E[b'_{V}(A_0,O_0)\mid A_0,S_0]\mid O^{-}_0,A_0 ] \tag{Definition of bridge functions}\\\
     &=\E[\E[b'_{V}(A_0,O_0)\mid S_0,O^{-}_0 ,A_0]\mid O^{-}_0,A_0]   \tag{$O_0 \perp O^{-}_0 \mid S_0,A_0 $ }\\\
     &=\E[b'_{V}(A_0,O_0)\mid O^{-}_0,A_0 ]. 
\end{align*}

Next, we prove weight bridge functions are learnable weight bridge functions: 
\begin{align*}
    &\E[b'_W(A_0,O^{-}_0) \mid A_0,O_0 ]= \E[\E[b'_W(A_0,O^{-}_0)\mid A_0,O_0,S_0 ] \mid A_0,O_0 ]\\
    &=  \E[\E[b'_W(A_0,O^{-}_0)\mid A_0,S_0 ] \mid A_0,O_0 ] \tag{$O_0 \perp O^{-}_0  \mid A_0,S_0 $}\\
    &=\E[1/\pi^b(A_0\mid S_0)\mid A_0,O_0 ]  \tag{Definition of bridge functions}\\
 &=\E[1/\pi^b(A_0\mid S_0,O_0)\mid A_0,O_0 ]  \tag{$A_0 \perp O_0 \mid S_0$}\\
    &=1/P_{\pi_b}(A_0\mid O_0). 
\end{align*}
\end{proof}


\begin{proof}[Proof of \pref{lem:some_characterization}]

%We first shows that $\E[b_W(A_0,O^{-}_0)\mid A_0,O_0]=1/\pi^b(A_0\mid O_0)$ implies 
First, note
 $$\E[\sum_a f(O_0,a)-b_W(A_0,O^-_0)f(O_0,A_0)]=0,\quad \forall f:\Ocal\times \Acal \to \RR,$$
is equivalent to 
$$\E[f(O_0,a)-b_W(A_0,O^-_0)\mathrm{I}(A_0=a)f(O_0,a)]=0,\quad \forall f:\Ocal\times \Acal \to \RR,\forall a\in \Acal.$$
This condition is equivalent to 
\begin{align*}
    \E[f(O_0,a)\{1-b_W(A_0,O^-_0)\pi^b(a_0\mid O_0)\}]=0,\quad \forall f:\Ocal\times \Acal \to \RR.
\end{align*}
This is equivalent to $b_W(A_0,O^-_0)\pi^b(a_0\mid O_0)=1$. 


\end{proof}

\begin{proof}[Proof of \pref{thm:final_step}]
We prove the importance sampling formula. Let $b'_V$ be a reward bridge function and $b_W$ be an learnable bridge function. 
Then,
\begin{align*}
        J(\epol)&= \E[\sum_a b'_V(a,O_0)]=\E[1/P_{\bpol}(A_0\mid O_0) b'_V(A_0,O_0) ] \tag{Result of \pref{lem:first_step}}\\
        &= \E[\E[b_W(A_0,O^{-}_0) \mid A_0,O_0] b'_V(A_0,O_0) ] \tag{Definition} \\ 
     &= \E[b_W(A_0,O^{-}_0) b'_V(A_0,O_0) ]\\ 
        &= \E[b_W(A_0,O^{-}_0)  \E[b'_V(A_0,O_0)\mid A_0,S_0] ] \\
        &=\E[b_W(A_0,O^{-}_0)\E[R_0\epol(A_0\mid O_0)\mid A_0,S_0] ] \tag{Definition}\\
        &= \E[b_W(A_0,O^{-}_0)R_0\epol(A_0\mid O_0)]. 
\end{align*}

We prove the value function based formula. Let $b'_W$ be a weight bridge function and $b_V$ be an learnable weight bridge function. Then, 
\begin{align*}
    J(\epol)&=\EE[b'_W(A_0,O^{-}_0)R_0\pi^e(A_0\mid O_0)]=\EE[b'_W(A_0,O^{-}_0)\E[R_0\pi^e(A_0\mid O_0)\mid A_0,O^{-}_0]] \tag{Result of \pref{lem:first_step}}\\ 
      &= \EE[b'_W(A_0,O^{-}_0)b_V(A_0,O_0)] \tag{Definition}\\
       &= \EE[\E[b'_W(A_0,O^{-}_0)\mid A_0,S_0 ]b_V(A_0,O_0)] \\
        &= \EE[1/\pi^b(A_0\mid S_0) b_V(A_0,O_0)] \tag{Definition}\\
        &=\E[\sum_a b_V(a,O_0) ]. 
\end{align*}

\end{proof}


\begin{proof}[Proof of \pref{thm:final_step_plus}]
\begin{align*}
        J(\epol) & = \E[ (1/P_{\pi_b}(A_0 \mid S_0 )R_0\epol(A_0\mid O_0)] \\ 
               & = \E[ (1/P_{\pi_b}(A_0 \mid S_0 ) \E[R_0\epol(A_0\mid O_0)\mid A_0,S_0)]] \\ 
              & = \E[ (1/P_{\pi_b}(A_0 \mid S_0 ) \E[b_V(A_0,O_0)\mid A_0,S_0)]] \tag{Completeness} \\ 
                &= \E[\sum_a b_V(a,O_0) ].
\end{align*}


\end{proof}

\subsubsection{Discrete setting}

\cite{tennenholtz2020off}  assume the following. 
\begin{assum}\label{asm:strong}
$\Prr(\bO_0 \mid A_0=a,\bO^{-}_0),\Prr(\mathbf{S}_0\mid A_0=a,\bO^{-}_0)$ are invertible. 
\end{assum}
This implies $|\bS|=|\bO|$, which is very strong. Remark this is also assumed in the paper which proposed negative controls \cite{miao2018identifying}. Instead, we require the following weaker assumption: 
\begin{assum}\label{asm:weak2}
$\rank(\Prr(\bO_0\mid \bS_0))=|\Scal|$ and $\rank(\Sbb_0 \mid \Ob_0,A_0=a))=|\Scal|$. 
\end{assum}
The first assumption ensure the existence of weight bridge functions. The second assumption ensures the completeness assumption. 
We show this is equivalent to the assumption in  \cite{nair2021spectral}:
\begin{assum}
\label{asm:weak3}
$\rank(\Prr(\bO_0 \mid A_0=a,\bO^{-}_0))= |\Scal|$. 
\end{assum}


\begin{proof}[Proof of \pref{lem:equivalence}]
Assumption \pref{asm:weak3} implies Assumption \pref{asm:weak2} since 
\begin{align*}
    |\Scal|= \rank(\Prr(\mathbf{O}_0 \mid A_0=a,\bO^{-}_0))\leq    \min( \rank( \Prr(\mathbf{O}_0 \mid A_0=a,\bS_0)), \rank(\Prr(\bS_0 \mid A_0=a,\bO^{-}_0))). 
\end{align*}
Then, Assumption \pref{asm:weak3} is concluded. 

Assumption \pref{asm:weak2} implies assumption \pref{asm:weak3} from Sylvester’s rank inequality:
\begin{align*}
 |\Scal| &=\rank( \Prr(\mathbf{O}_0 \mid A_0=a,\bS_0)) \tag{From Assumption \pref{asm:weak2}} \\
%  &= \rank( \Prr(\mathbf{O}_0 \mid A_0=a,\bS_0))+ \rank(\Prr(\bO^{-}_0 \mid A_0=a, \bS_0 ))-|\Scal| \tag{From Assumption \pref{asm:weak2}}\\ 
 &=\rank( \Prr(\mathbf{O}_0 \mid A_0=a,\bS_0))+ \rank(\Prr(\bS_0 \mid A_0=a,\bO^{-}_0))-|\Scal| \tag{See argument above}\\
&\leq \rank( \Prr(\mathbf{O}_0 \mid A_0=a,\bS_0)\Prr(\bS_0 \mid A_0=a,\bO^{-}_0)) \tag{ Sylvester’s rank inequality:}\\
&= \rank(\Prr(\mathbf{O}_0 \mid A_0=a,\bO^{-}_0)).
\end{align*}
Besides,
\begin{align*}
\rank(\Prr(\mathbf{O}_0 \mid A_0=a,\bO^{-}_0))\leq    \min( \rank( \Prr(\mathbf{O}_0 \mid A_0=a,\bS_0)), \rank(\Prr(\bS_0 \mid A_0=a,\bO^{-}_0)))=|\Scal|. 
\end{align*}
Thus, 
\begin{align*}
    \rank(\Prr(\mathbf{O}_0 \mid A_0=a,\bO^{-}_0))=|\Scal|. 
\end{align*}
\end{proof}

We finally remark the existence of weight bridge functions is equal to the one 
\begin{assum}
Suppose  $P_{\bpol}(O^-_0= o^{-} \mid A_0=a)>0, P_{\bpol}(S_0=s\mid A_0=a)>0$ for any $o^- \in \Ocal, s\in \Scal,a\in \Acal$. Then, 
%%%\label{asm:weak3}
$\rank(\Prr(\bO_0 \mid \bS_0))= |\Scal|$ and $\rank(\Prr(\bS_0 \mid A_0=a.\bO^{-}_0))= |\Scal|$ are equivalent. 
\end{assum}
\begin{proof}
We have 
\begin{align*}
    \{\Prr(\bS_0 \mid A_0=a,\bO^{-}_0)\}^{\top}=\Lambda_1 \Prr(\bO^{-}_0 \mid A_0=a,\bS_0)\Lambda_2 
\end{align*}
where $\Lambda_1$ is a $|\Ocal| \times |\Ocal|$ matrix s.t. $(i,i)$-th element is $1/P_{\bpol}(O^-_0= o^{-} \mid A_0=a) $ and $\Lambda_2 $ is a $|\Scal|\times |\Scal|$ matrix s.t. $(i,i)$-th element is $P_{\bpol}(S_0=s\mid A_0=a)$.  
Thus, $\rank(\Prr(\bO^{-}_0 \mid \bS_0))=\rank(\Prr(\bO^{-}_0 \mid A_0=a,\bS_0))=\rank(\Prr(\bS_0 \mid A_0=a, \bO^{-}_0)) \geq |\Scal|$.  
\end{proof}

Finally, we give the identification formula:  

\begin{proof}[Proof of \pref{thm:discrete_identify}]
We have
\begin{align*}
    \Pr(\bO_0 \mid \bO^{-}_0, a)   =      \Pr(\bO_0 \mid \bS_0, a) \Pr(\bS_0\mid \bO^{-}_0, a),\quad \Pr(r, o \mid \bO^{-}_0,a)  =     \Pr(r,o \mid \bS_0,a) \Pr(\bS_0\mid \bO^{-}_0, a). 
\end{align*}
Let the SVD decomoposition of $  \Pr(\bO_0 \mid \bO^{-}_0, a) $ be $ABC$, where $A$ is a $|\Ocal|\times |\Scal|$ matrix, $B$ is a $ |\Scal|\times |\Scal|$ matrix, and $C$ is a $|\Scal|\times |\Ocal|$ matrix. 
\begin{align*}
    \mathrm{I}= A^{\top}\Pr(\bO_0 \mid \bO^{-}_0, a)C^{\top}B^{-1}=A^{\top}\Pr(\bO_0 \mid \bS_0, a)\Pr(\bS_0 \mid \bO^{-}_0,a )C^{\top}B^{-1}. 
\end{align*}
Therefore, we have
\begin{align*}
   A^{\top} \Pr(\bO_0 \mid \bS_0 )=\{ \Pr(\bS_0 \mid \bO^{-}_0,a )C^{\top}B^{-1}\}^{-1}. 
\end{align*}
noting $ \Pr(\bS_0 \mid \bO^{-}_0,a) C^{\top}B^{-1} $ is full-rank matrix from the assumption.  

In addition, we have 
\begin{align}\label{eq:minor}
 \Pr(r,o \mid \bO^{-}_0,a) C^{\top}B^{-1} = \Pr(r,o  \mid \bS_0,a)  \Pr(\bS_0\mid \bO^{-}_0, a)C^{\top}B^{-1}. 
\end{align}

Thus, 
\begin{align*}
 \Pr(r,o  \mid \bS_0,a) &= \Pr(r,o  \mid \bO^{-}_0,a) C^{\top}B^{-1}\{\Pr(\bS_0\mid \bO^{-}_0, a)C^{\top}B^{-1}\}^{-1} \tag{From \pref{eq:minor}} \\ 
   &=  \Pr(r,o  \mid \bO^{-}_0,a) C^{\top}B^{-1}A^{\top}\Pr(\bO_0 \mid \bS_0, a)\\
   &= \Pr(r,o  \mid \bO^{-}_0,a)\{ \Pr(\bO_0 \mid \bO^{-}_0, a)\}^{+}\Pr(\bO_0 \mid \bS_0). 
\end{align*}
Besides, 
\begin{align*}
    J &=\sum_{a,r,o,s} r p(r,o \mid s,a)\epol(a\mid o)p(s) \tag{Definition} \\
       &=\sum_{a,r,o,s}   \Pr(r,o  \mid \bO^{-}_0,a)\{ \Pr(\bO_0 \mid \bO^{-}_0, a)\}^{+}\Pr(\bO_0 \mid s)\epol(A \mid O)p(s) \\
      &=\sum_{a,r,o}r\epol(a\mid o) \Pr(r ,o \mid \bO^{-}_0,a)\{ \Pr(\bO_0 \mid \bO^{-}_0, a)\}^{+}\Pr(\bO_0). 
\end{align*}

\end{proof}


\subsection{ Proof of  Section \ref{subsec:identify_homo}   }


We define $Q(s,a)\coloneqq \E[b'_V(a,O) \mid A=a,S=s]$. We show this $Q(s,a)$ satisfies a recursion formula. 

\begin{lemma}\label{lem:value2}
 \begin{align*}
         Q(S,A)&=\E[R \epol(A\mid O)\mid A,S]+  \gamma\E\bracks{\sum_{a'}Q(S^{+},a')\epol(A \mid O) \mid A,S}. 
 \end{align*}
\end{lemma}
\begin{proof}[Proof of Lemma \ref{lem:value2}]
From the definition, 
\begin{align*}
   Q(s,a)&=\E[R_0 \epol(a\mid O_0)\mid A_0=a,S_0=s]+  \E_{\epol}\bracks{\sum_{t=1}^{\infty} \gamma^t R_t\epol(a\mid O_0)\mid A_0=a,S_0=s}. 
 \end{align*}  
 Then, we have 
 \begin{align*}
    &\E_{\epol}\bracks{\sum_{t=1}^{\infty} \gamma^t R_t\epol(a\mid O_0)\mid A_0=a,S_0=s}\\
    &= \gamma\E\bracks{\sum_{a'}\E_{\epol}[\sum_{t=1}^{\infty} \gamma^{t-1} R_t\mid S_1,A_1=a']\epol(a'\mid O_1)\epol(a\mid O_0)\mid A_0=a,S_0=s}\\
  &= \gamma\E\bracks{\sum_{a'}\E_{\epol}[\sum_{t=1}^{\infty} \gamma^{t-1} R_t\mid S_1,A_1=a']\E[\epol(a'\mid O_1)\mid S_1,A_1=a']\epol(a\mid O_0)\mid A_0=a,S_0=s}\\
    &= \gamma\E\bracks{\sum_{a'}\E_{\epol}[\sum_{t=1}^{\infty} \gamma^{t-1} R_t\epol(a'\mid O_1)\mid S_1,A_1=a']\epol(a\mid O_0)\mid A_0=a,S_0=s} \tag{$R_1,\cdots, R_{H-1}\perp O_1\mid S_1,A_1  $}\\
    &= \gamma\E\bracks{\sum_{a'}Q^{\epol}(a',S_1)\epol(a\mid O_0) \mid A_0=a,S_0=s}. 
\end{align*}
In conclusion, 
 \begin{align*}
    Q(S,A)=\E[R \epol(a\mid O)\mid A,S]+  \gamma\E\bracks{\sum_{a'}Q(S^{+},a')\epol(A \mid O) \mid A,S}. 
 \end{align*}
\end{proof}

By using the above lemma, we show learnable reward bridge functions are reward bridge functions. This is a part of the statement in \pref{thm:key_rl}. 

\begin{lemma}[Learnable reward bridge functions are reward bridge functions]\label{lem:v_recursive}
\begin{align*}
   \E[b'_{V}(A,O)\mid A,O^{-}] &=\E[R \epol(a\mid O)\mid A,O^{-}]+  \gamma\E\bracks{\sum_{a'}b'_{V}(a',O^{+})\epol(A \mid O) \mid  A,O^{-}}. 
 \end{align*}
\end{lemma}
\begin{proof}
From \pref{lem:value2}, we have 
  \begin{align*}
   \E[b'_{V}(A,O)\mid S,A] &=\E[R \epol(a\mid O)\mid A,S]+  \gamma\E\bracks{\sum_{a'}\E[b'_{V}(a',O^{+})|S^{+}]\epol(A \mid O) \mid A,S}\\
    &=\E[R \epol(a\mid O)\mid A,S]+  \gamma\E\bracks{\sum_{a'}b'_{V}(a',O^{+})\epol(A \mid O) \mid A,S}. 
 \end{align*}
Then, from $O,R,O^{+}\perp O^{-} \mid S,A$, we have
\begin{align*}
&\E[\E[b'_{V}(A,O)\mid S,A]|A, O^{-}] =    \E[\E[b'_{V}(A,O)\mid S,A,O^{-}]|A,O^{-}]= \E[b'_{V}(A,O)\mid A,O^{-}]\\ 
&\E[\E[R \epol(A\mid O)\mid A,S]|A,O^{-}]  = \E[\E[R \epol(A\mid O)\mid A,S,O^{-}]|A,O^{-}]=\E[R \epol(A\mid O)\mid A,O^{-}]\\
&\E\bracks{\bracks{\sum_{a'}b'_{V}(a',O^{+})\epol(A \mid O) \mid A,S}\mid A,O^-}=\E\bracks{\sum_{a'}b'_{V}(a',O^{+})\epol(A \mid O) \mid  A,O^{-}} . 
 \end{align*}
In conclusion,  
\begin{align*}
   \E[b'_{V}(A,O)\mid A,O^{-}] &=\E[R \epol(A\mid O)\mid A,O^{-}]+  \gamma\E\bracks{\sum_{a'}b'_{V}(a',O^{+})\epol(A \mid O) \mid  A,O^{-}}. 
 \end{align*}
 
\end{proof}

Next, we show learnable weight bridge functions are action bridge functions. This is a part of the statement in \pref{thm:key_rl}. 
Here, letting $w(s)= d_{\epol}(s)/b(s)$, recall 
\begin{align}\label{eq:previous_key}
    \E\bracks{\gamma w(S)\frac{\epol(A|O)}{\bpol(A|S)}f(S')- w(S)f(S) }+(1-\gamma)\E_{\tilde S\sim \nu}[f(\tilde S)]=0,\,\forall f:\Scal \to \RR 
\end{align}
from \citet[Lemma 16 ]{KallusNathan2019EBtC} which is a modification of the lemma in \cite{Liu2018}. Recall $\nu$ is an initial distribution. 

\begin{lemma}[Learnable weight bridge functions are weight bridge functions.]\label{lem:learnable_action}
\begin{align*}
    \E\bracks{\gamma  b'_{W}(A,O^{-})\epol(A|O)f(O^{+},a')-\rI(A=a')b'_{W}(A,O^{-}) f(O,A) }+(1-\gamma)\E_{\tilde O\sim \nu_{\Ocal}}[f(\tilde O,a')]=0,\,\forall f:\Scal\to \RR. 
\end{align*}
Similarly, 
\begin{align*}
    \E\bracks{\sum_{a'\in \Acal}\gamma  b'_{W}(A,O^{-})\epol(A|O)f(O^{+},a')-b'_{W}(A,O^{-}) f(O,A) }+(1-\gamma)\E_{\tilde O\sim \nu_{\Ocal}}[\sum_{a'\in \Acal} f(\tilde O,a')]=0,\,\forall f:\Scal\to \RR.  
\end{align*}

\end{lemma}
\begin{proof}
We first prove the first statement: 
\begin{align*}
     & \E\bracks{\gamma  b'_{W}(A,O^{-})\epol(A\mid O) f(O^{+},a')-\rI(A=a') b'_{W}(A,O^{-}) f(O,A) }\\
    &=\E\bracks{\gamma  \E[b'_{W}(A,O^{-})\mid A,S,O^{+},O ]\epol(A\mid O) f(O^{+},a')-\rI(A=a')\E[b'_{W}(A,O^{-})\mid A,S, O]f(O,A) }\\
     &=\E\bracks{\gamma \E[b'_{W}(A,O^{-})\mid A,S  ] \epol(A\mid O) f(O^{+},a')-\rI(A=a')\E[b'_{W}(A,O^{-})\mid A,S ]f(O,A) }\\
    &=\E\bracks{\gamma w(S)/\bpol(A\mid S)\epol(A|O)f(O^{+},a')-w(S)\rI(A=a')/\bpol(A\mid S) f(O,A) } \tag{Definition}\\    
    &=\E\bracks{\gamma w(S)/\bpol(A\mid S)\epol(A|O)\E[f(O^{+},a')\mid S^{+},A,O,S]-w(S)\rI(A=a')/\bpol(A\mid S)\E[f(O,A)\mid S,A=a'] }\\  
    &=\E\bracks{\gamma w(S)\epol(A|O)/\bpol(A\mid S)\E[f(O^{+},a')\mid S^{+}]-w(S)\E[f(O,a')\mid S] }\\
    &= -(1-\gamma)\E_{S\sim \nu}[\E[f(\tilde O,a')\mid S]] \tag{From \pref{eq:previous_key}}\\
    &=  - (1-\gamma)\E_{\tilde O\sim \nu_{\Ocal}}[f(\tilde O,a')]. 
\end{align*}
The second statement is proved by taking summation over the action space. 
\end{proof}

Finally, we show if bridge functions exist, we can identify the policy value. Before proceeding, we prove the following helpful lemma. 
\begin{lemma}[Identification formula with (unlearnable) bridge functions ]\label{lem:fake_identification}
Assume the existence of bridge functions. Then, let $b'_V,b'_W$ be any bridge functions. Then, we have 
\begin{align*}
       J(\epol)= \E_{\tilde O\sim \nu_{\Ocal}}[\sum_a b'_V(a,\tilde O)],\quad     J(\epol)=(1-\gamma)^{-1}\E[b'_W(A,O^-)R\epol(A\mid O)]. 
\end{align*}
\end{lemma}
\begin{proof}
The first formula is proved as follows:
\begin{align*}
    & \E_{\tilde O\sim \nu_{\Ocal}}[\sum_a b'_V(a,\tilde O)]=\E_{S\sim \nu }[\E[\sum_a b'_V(a,\tilde O)\mid S]]=\E_{S\sim \nu }[\E[\sum_a b'_V(a,\tilde O)\mid A=a,S]]\\
    &=\E_{S_0\sim \nu }[\E[\sum_a b'_V(a,\tilde O_0)\mid A_0=a,S_0]]\\
  &=  \E_{S_0\sim \nu}[\sum_{a}    \E_{\epol}[\sum_{t=0}^{\infty} \gamma^t R_t\epol(a\mid O_0)|A_0=a,S_0]] \tag{Definition}\\
    &=  \E_{S_0\sim \nu}[\sum_{a}    \E_{\epol}[\E_{\epol}[\sum_{t=0}^{\infty}  \gamma^t R_t\mid A_0=a,S_0,O_0]\epol(a\mid O_0)|A_0=a,S_0]] \\
       &=  \E_{S_0\sim \nu}[\sum_{a}    q^{\epol}(S_0,a)\E_{\epol}[\epol(a\mid O_0)|A_0=a,S_0]]\\
            &=  \E_{S_0\sim \nu}[\sum_{a}    q^{\epol}(S_0,a)\E_{\epol}[\epol(a\mid O_0)|S_0]]=  \E_{S_0\sim \nu}[\sum_{a}    q^{\epol}(S_0,a)\epol(a\mid O_0)]\\
            &=J(\epol).
\end{align*}
Here, we define $\E_{\epol}[\sum_{t=0}^{\infty} \gamma^t R_t|A_0=a,S_0=s]=q^{\epol}(a,s)$.

The second formula is proved as follows: 
\begin{align*}
\E[b'_{W}(A, O^{-})R\epol(A\mid O)]&= \E[\E[b'_{W}(A, O^{-})\mid A,S,R,O]\epol(A\mid O)R] \\
&= \E[\E[b'_{W}(A, O^{-})\mid A,S]\epol(A\mid O)R] \tag{ $ O^- \perp R,O \mid S,A $} \\
&=\E\bracks{\frac{w(S)}{\bpol(A|S)} \epol(A\mid O)R} \tag{Definition}\\
&=J(\epol). 
\end{align*}
\end{proof}

We are ready to give the proof of the final identification formula \pref{thm:key_rl}. The statement is as follows. 

\begin{theorem}\label{thm:final_rl_ape}
Assume the existence of bridge functions. Let $b_V,b_W$ be any learnable bridge functions. 
Then, 
\begin{align*}
      J(\epol)=\E_{\tilde O\sim \nu_{\Ocal}}[\sum_{a'} b_V(\tilde O,a')],\quad    J(\epol)=(1-\gamma)^{-1}\E[b_W(A,O^-)R\epol(A\mid O)]. 
\end{align*}
\end{theorem}
\begin{proof}
First, we prove the first formula. This is concluded by 
\begin{align*}
    J(\epol)&= (1-\gamma)^{-1}\E[b'_W(A,O^{-})R\epol(A\mid O)] \tag{From \pref{lem:fake_identification}}\\
     &= (1-\gamma)^{-1}\E[b'_W(A,O^{-})\E[R\epol(A\mid O)\mid A,O^-]]\\
     &=(1-\gamma)^{-1} \E\bracks{b'_W(A,O^{-})\E\bracks{\gamma \sum_{a'} b_V(a',O^+)\epol(A\mid O)-b_V(A,O) \mid A,O^-}} \tag{$b'_W$ is also an learnable action bridge function. }\\
     &=\E_{\tilde O\sim \nu_{\Ocal}}[\sum_{a'} b_V(\tilde O,a')].    \tag{From \pref{lem:learnable_action}}
\end{align*}

Next, we prove the second formula. This is concluded by 
\begin{align*}
    J(\epol) &= \E_{\tilde O\sim \nu_{\Ocal}}[\sum_{a'} b'_V(\tilde O,a')] \tag{From \pref{lem:fake_identification}} \\
        &= (1-\gamma)^{-1}\E\bracks{b_W(A,O^{-})\E\bracks{\gamma \sum_{a'} b'_V(a',O^+)\epol(A\mid O)-b'_V(A,O) \mid A,O^-}} \tag{Definition of $b_W$}\\
        &=(1-\gamma)^{-1}\E[b_W(A,O^{-})\E[R\epol(A\mid O)\mid A,O^-]] \tag{$b'_V$ is also an learnable reward function.} \\ 
        &= (1-\gamma)^{-1}\E[b_W(A,O^{-})R\epol(A\mid O)]. 
\end{align*}
\end{proof}


\begin{proof}[Proof of \pref{thm:without0}]

By the assumption $O,R,O^+ \perp O^- \mid S,A$ we see any $b_V$ satisfies
\begin{align*}
    \EE\bracks{\EE\bracks{\gamma \sum_{a'}b_V(a',O^+) +R\epol(A\mid O)-b_V(A,O)\mid S,A}\mid A,O^-}=0.  
\end{align*}
From the completeness assumption, 
\begin{align}\label{eq:result_comp}
    \EE\bracks{\gamma \sum_{a'}b_V(a',O^+) +R\epol(A\mid O)-b_V(A,O)\mid S,A}=0. 
\end{align}
Thus, we have 
\begin{align*}
    J(\epol)&= (1-\gamma)^{-1}\E[w(S) \epol(A\mid O)/P_{\pi_b}(A\mid S) R] \\
     &= (1-\gamma)^{-1}\E[w(S) /P_{\pi_b}(A\mid S)  \E[R\epol(A\mid O)\mid A,S ]]\\
  &= (1-\gamma)^{-1}\E\bracks{w(S) /P_{\pi_b}(A\mid S)   \EE\bracks{\gamma \sum_{a'}b_V(a',O^+) +R\epol(A\mid O)-b_V(A,O)\mid S,A}}+\E_{\tilde O\sim \nu_{\Ocal}}[\sum_{a'} b_V(\tilde O,a')]\\
     &=\E_{\tilde O\sim \nu_{\Ocal}}[\sum_{a'} b_V(\tilde O,a')].    \tag{From \pref{eq:result_comp}}
\end{align*}

\end{proof}


\subsection{Proof of Section \ref{subsec:theory_value}}

\begin{proof}[Proof of \pref{thm:con_results}]
By simple algebra, the estimator is written as 
\begin{align*}
   \hat b_V= \inf_{f\in \Vcal}\sup_{g\in \Vcal^{\dagger}}\E_{\Dcal}[(\Zcal f)^2]- \E_{\Dcal}[(\Zcal f-g(A,O^-))^2] 
\end{align*}
where $\Zcal f=R\epol(A \mid O)+\sum_{a'}f(a',O^+)\epol(A\mid O)$. In this proof, we define
\begin{align*}
   \bar C= \max(C_{\Vcal},C_{\Vcal^{\dagger}}, 1). 
\end{align*}
Furthermore, $c$ is some universal constant.   

\paragraph{Show the convergence of inner maximizer}

For fixed $f\in \Vcal$, we define 
\begin{align*}
    \hat g_f=\sup_{g\in \Vcal^{\dagger}}- \E_{\Dcal}[(\Zcal f-g(A,O^-))^2], 
\end{align*}
we want to prove with probability $1-\delta$: 
\begin{align*}
  \forall f\in \Vcal:  |\E_{\Dcal}[(\Zcal f-\hat g_f(A,O^-))^2]-\E_{\Dcal}[(\Zcal f-\Tcal f)^2(A,O^-)]|\leq \frac{c \log(|\Vcal||\Vcal^{\dagger}|c/\delta)}{n}. 
\end{align*}
Note since $\Bcal f$ is the Bayes optimal regressor, we have 
\begin{align}\label{eq:regressor}
    \E[(\Zcal f-\Tcal f(A,O^-))^2-(\Zcal f-g(A,O^-))^2]=\E[(\Tcal f-g(A,O^-))^2 ]. 
\end{align}
Hereafter, to simplify the notation, we often drop $(A,O^-)$. Then, from Bernstein's inequality, with probability $1-\delta$, 
\begin{align}\label{eq:uniform}
  \forall f\in \Vcal,\forall  g\in \Vcal^{\dagger}:  |\{\E_{\Dcal}-\E\}[(\Zcal f-\Tcal f)^2-(\Zcal f-g)^2]|\leq c \bar C\sqrt{\frac{\E[(\Tcal f-g)^2] \log(|\Vcal||\Vcal^{\dagger}|c/\delta)}{n}}+\frac{c \bar C^2\log(|\Vcal||\Vcal^{\dagger}|c/\delta)}{n}.
\end{align}
Hereafter, we condition on the above event. In addition, from Bellman closedness assumption $\Tcal \Vcal\subset \Vcal^{\dagger}$, 
\begin{align*}
    \E_{\Dcal}[(\Zcal f-\hat g_f)^2-(\Zcal f-\Tcal f)^2]\leq 0. 
\end{align*}
Then, 
\begin{align*}
  \E[(\Tcal f-\hat g_f)^2 ]&=\E[(\Zcal f-\Tcal f)^2-(\Zcal f-\hat g_f)^2] \\
  &\leq |\{\E_{\Dcal}-\E\}[(\Zcal f-\Tcal f)^2-(\Zcal f-\hat g_f)^2]|+\E_{\Dcal}[(\Zcal f-\hat g_f)^2-(\Zcal f-\Bcal f)^2] \\
  &\leq  |\{\E_{\Dcal}-\E\}[(\Zcal f-\Tcal f)^2-(\Zcal f-\hat g_f)^2]| \\
  &\leq c \bar C\sqrt{\frac{\E[(\Tcal f-\hat g_f)^2] \log(|\Vcal||\Vcal^{\dagger}|c/\delta)}{n}}+\frac{c \bar C^2\log(|\Vcal||\Vcal^{\dagger}|c/\delta)}{n}. \tag{From \pref{eq:uniform}}
\end{align*}
This concludes
\begin{align*}
      \E[(\Tcal f-\hat g_f)^2 ]\leq c\mathrm{Error},\quad \mathrm{Error}\coloneqq  \frac{ \bar C^2\log(|\Vcal||\Vcal^{\dagger}|c/\delta)}{n}.
\end{align*}
Then,  
\begin{align*}
 |\E_{\Dcal}[(\Zcal f-\hat g_f)^2]-\E_{\Dcal}[(\Zcal f-\Tcal f)^2]|    & \leq \E[(\Zcal f-\Tcal f)^2-(\Zcal f-\hat g_f)^2]+ c\mathrm{Error} \tag{ From \pref{eq:uniform}}\\
    & = \E[(\Tcal f-\hat g_f)^2 ]+ c\mathrm{Error} \tag{From \pref{eq:regressor}}\\
    &\leq 2c\mathrm{Error}. 
\end{align*}

\paragraph{Show the convergence of outer minimizer}

From the first observation, we can see
\begin{align*}
    \E_{\Dcal}[(\Zcal \hat b_V)^2-(\Zcal \hat b_V-\Tcal\hat b_V(A,O^-))^2 ]\leq  \E_{\Dcal}[(\Zcal b_V)^2-(\Zcal b_V-\Tcal b_V(A,O^-))^2 ]+c\mathrm{Error}. 
\end{align*}
%Thus, we can treat as if the loss function was
%\begin{align*}
%        \E_{\Dcal}[(\Zcal f-f)^2-(\Zcal f-\Bcal f)^2 ] 
%\end{align*}
%up to some errors quantified by $\mathrm{Error}$.
Note 
\begin{align*}
    \E[(\Zcal f)^2-(\Zcal f-\Tcal f(A,O^-))^2-\{(\Zcal b_V)^2-(\Zcal b_V-\Tcal b_V(A,O^-))^2\} ]= \E[(\Tcal f)(A,O^-)^2] 
\end{align*}
Here,  from Bernstein's inequality, with probability $1-\delta$, 
\begin{align*}
    \forall f\in \Vcal, &(\E_{\Dcal}-\E)[(\Zcal f)^2-(\Zcal f-\Bcal f)^2-\{(\Zcal b_V)^2-(\Zcal b_V-\Bcal b_V)^2\} ]\\
     &\leq \bar C\sqrt{\E[(\Tcal f)^2(A,O^-)] \frac{ \log(|\Vcal|/\delta)}{n} }+\frac{\bar C^2\log(|\Vcal|/\delta)}{n}. 
\end{align*}
Hereafter, we condition on the above event. Then, 
\begin{align*}
    \E[(\Bcal \hat b_V-\hat b_V)^2]&= \E[(\Zcal \hat b_V)^2-(\Zcal \hat b_V-\Tcal \hat b_V)^2-\{(\Zcal b_V)^2-(\Zcal b_V-\Tcal b_V)^2\} ]\\
    &\leq (\E_{\Dcal}-\E)[(\Zcal \hat b_V)^2-(\Zcal \hat b_V- \Tcal \hat b_V)^2-\{(\Zcal b_V)^2-(\Zcal b_V-\Tcal b_V)^2\} ] \\ 
    & + \E_{\Dcal}[(\Zcal \hat b_V)^2-(\Zcal \hat b_V-\Bcal\hat b_V)^2-\{(\Zcal b_V)^2-(\Zcal b_V-\Tcal b_V)^2\} ]\\
    &\leq  \bar C\sqrt{\E[(\Tcal \hat b_V)^2(A,O^{-})] \frac{ \log(|\Vcal|c/\delta)}{n} }+\frac{\bar C^2\log(|\Vcal|c/\delta)}{n}+c\mathrm{Error}.  
\end{align*}
This concludes
\begin{align*}
      \E[(\Tcal \hat b_V)^2(A,O^{-})]\leq c\mathrm{Error}. 
\end{align*}
\end{proof}





\begin{proof}[Proof of \pref{thm:final_policy}]

~
\paragraph{First Statement}
Recall 
\begin{align*}
        J(\epol)=  \E[b_W(A,O^{-})\E[R\epol(A\mid O)\mid A,O^-] 
\end{align*}
from \pref{thm:final_rl_ape} and the existence of $b_W$. 
Furthermore, 
\begin{align*}
   &(1-\gamma)\E_{\tilde O\sim \nu_{\Ocal}}[\sum_{a'} \hat b_V(\tilde O,a')]  \\
   &=  \E\bracks{b_W(A,O^{-})\E\bracks{\gamma \sum_{a'} \hat b_V(a',O^+)\epol(A\mid O)-\hat b_V(A,O) \mid A,O^-}}.  \tag{$b_W$'s are also observe bridge functions form \pref{thm:key_rl}}
\end{align*}
Thus, this concludes 
\begin{align*}
   & J(\epol)-\E_{\tilde O\sim \nu_{\Ocal}}[\sum_{a'} \hat b_V(\tilde O,a')]\\
     &=(1-\gamma)^{-1}\E\bracks{b_W(A,O^{-})\E\bracks{\gamma \sum_{a'} \hat b_V(a',O^+)\epol(A\mid O)+R\epol(A\mid O)-\hat b_V(A,O) \mid A,O^-}}\\
     &= (1-\gamma)^{-1}\E\bracks{b_W(A,O^{-}) \Tcal \hat b_V (A,O^-)}. 
\end{align*}
Then, from CS inequality, we have
\begin{align*}
    |J(\epol)-\E_{\tilde O\sim \nu_{\Ocal}}[\sum_{a'} \hat b_V(\tilde O,a')]|\leq (1-\gamma)^{-1}\E[b_W(A,O^{-})^2]^{1/2} \E[\{\Tcal \hat b_V(A,O^-)\}^2 ]^{1/2}. 
\end{align*}
This concludes the final statement. 
\end{proof}

\begin{proof}[Proof of \pref{thm:final_policy_comp}]
Recall 
\begin{align*}
        J(\epol)=  \E[ w(S)/P_{\pi_b}(A\mid S)\E[R\epol(A\mid O)\mid A,S]] 
\end{align*}
Furthermore, 
\begin{align*}
   &(1-\gamma)\E_{\tilde O\sim \nu_{\Ocal}}[\sum_{a'} \hat b_V(\tilde O,a')]  \\
   &=  \E\bracks{w(S)/P_{\pi_b}(A\mid S) \E\bracks{\gamma \sum_{a'} \hat b_V(a',O^+)\epol(A\mid O)-\hat b_V(A,O) \mid A,S}}. 
\end{align*}
Thus, this concludes 
\begin{align*}
   & J(\epol)-\E_{\tilde O\sim \nu_{\Ocal}}[\sum_{a'} \hat b_V(\tilde O,a')]\\
     &=(1-\gamma)^{-1} \E\bracks{w(S)/P_{\pi_b}(A\mid S) \E\bracks{\gamma \sum_{a'} \hat b_V(a',O^+)\epol(A\mid O) + R\epol(A\mid O)-\hat b_V(A,O) \mid A,S}}\\
     &= (1-\gamma)^{-1}\E\bracks{w(S)/P_{\pi_b}(A\mid S)  \Tcal_{S} \hat b_V (A,S) }. 
\end{align*}
Then, from CS inequality, we have
\begin{align*}
    |J(\epol)-\E_{\tilde O\sim \nu_{\Ocal}}[\sum_{a'} \hat b_V(\tilde O,a')]|\leq (1-\gamma)^{-1}\E[\{w(S)/P_{\pi_b}(A\mid S)\}^2]^{1/2} \E[  \Tcal_{S} \hat b_V (A,S)^2 ]^{1/2}. 
\end{align*}
Recalling $\E[  \{\Tcal_{S} \hat b_V (A,S)\}^2 ]\leq \kappa \E[  \{\Tcal \hat b_V (A,O^-)\}^2 ] $, this concludes the final statement. 



\end{proof}


\subsection{Proof of Section \ref{sec:theoryDRmethod}}

\begin{proof}[Proof of \pref{thm:dr_infinite}]
The first statement $J(\epol)=\E[J(f,b_V)]$ is proved by \pref{lem:learnable_action}:
\begin{align*}
    \E[J(f,b_V)] &= \E_{\tilde O\sim \nu_{\Ocal}}[\sum_a b_V(a,\tilde O)]+ \E\bracks{\frac{f(A,O^{-})}{1-\gamma}\{\{R+\gamma \sum_{a'}b_V(a',O^{+})\}\epol(A\mid O)-b_V(A,O)\}}\\ 
     &= \E_{\tilde O\sim \nu_{\Ocal}}[\sum_a b_V(a,\tilde O)] \tag{Definition of reward bridge functions}\\ 
     & =J(\epol).  \tag{From \pref{thm:final_rl_ape} }
\end{align*}

The second statement $J(\epol)=\E[J(b_W,f)]$ is proved by  \pref{lem:v_recursive}:
\begin{align*}
      \E[J(b_W,f)] &= \E_{\tilde O\sim \nu_{\Ocal}}[\sum_a f(a,\tilde O)]+ \E\bracks{\frac{b_W(A,O^{-})}{1-\gamma}\{\{R+\gamma \sum_{a'}f(a',O^{+})\}\epol(A\mid O)-f(A,O)\}}\\ 
      &= (1-\gamma)^{-1}  \E[R\epol(A\mid O)b_W(A,O^{-})  ] \tag{Definition of weight bridge functions} \\ 
      & =J(\epol).  \tag{From \pref{thm:final_rl_ape} }
\end{align*}
\end{proof}

\begin{proof}[Proof of  \pref{thm:cramer}]

Recall we have the observation: 
\begin{align*}
  Z=  \{O^{-},A,O,R,O^{+}\}. 
\end{align*}
We define 
\begin{align*}
    \tau_k =\prod_{t=1}^k \epol_t(a_t \mid o_t),\quad     \tau_{a:b} =\prod_{t=a}^b \epol_t(a_t \mid o_t). 
\end{align*}

From \cite{nair2021spectral,tennenholtz2020off}, the target functional is
{\small
\begin{align*}
    J=\sum_{k=0} \gamma^k \sum_{\mathfrak{j}_{r_k}}r_k \tau_k \Prr(r_k, o_k \mid a_k,\bO_{k-1})\{\Prr(\bO_k \mid a_k, \bO_{k-1}\}^{-1}\Prr(\bO_k,o_{k-1}\mid a_{k-1},\bO_{k-2})\{\Prr(\bO_{k-1} \mid a_{k-1}, \bO_{k-2})\}^{-1}\cdots \Prr(\bO_0). 
\end{align*}
}
We use the assumption $\rank(\Pr(\bO \mid A=a, \bO^{-}))=|\Scal|=|\Ocal|$, i.e., $\Pr(\bO \mid A=a, \bO^{-})$ is full-rank. 

We will show the existence of $\phi_{\mathrm{EIF}}(Z)$ s.t. 
\begin{align*}
     \nabla J(\theta) = \E[ \phi_{\mathrm{EIF}}(Z)\nabla \log P(Z)  ]. 
\end{align*}
Then, $\E[\phi_{\mathrm{EIF}}(Z)\phi^{\top}_{\mathrm{EIF}}(Z)] $ is the Cram\'er-Rao lower bound. 

Before the calculation, we introduce the bridge functions. Due to the assumptions, these are unique. By letting $\mathfrak{j}_{k}\coloneqq \{o_0, a_0, r_0, a_1, o_1, r_1, \cdots,r_k\}$, we define $b_{V}(a,o)$ as 
{\small
\begin{align*}
     b_{V}(a_0,o_0)=\sum_{k=0}^{\infty} \gamma^k \sum_{\mathfrak{j}_{r_k}\backslash (a_0,o_0) }r_k \tau_k \Prr(r_k, o_k \mid a_k,\bO_{k-1})\{\Prr(\bO_k \mid a_k, \bO_{k-1}\}^{-1}\cdots \{\Prr(\bO_{0} \mid a_{0}, \bO_{-1})\}^{-1} \rI(\bO_0=o_0). 
\end{align*}
}
Next, we define $b_{W}(a,o^{-})$. Recall 
\begin{align*}
    d^{\pi^e}_k(o_k)=\sum_{\mathfrak{j}_{o_k} \backslash o_k} \tau_{k-1} \rI(\bO_k=o_k)^{\top}\Prr(\bO_k,o_{k-1}\mid a_{k-1},\bO_{k-2})\{\Prr(\bO_{k-1} \mid a_{k-1}, \bO_{k-2})\}^{-1}\cdots \Prr(\bO_0). 
\end{align*}
where $\mathfrak{j}_{o_k}\coloneqq \{o_0, a_0, r_0, a_1, o_1, r_1, \cdots,o_k\}$. 
Then, we define $b_{W}(a,o^{-})$ as 
\begin{align*}
    b_{W}(a,o^-)=\frac{\rI(\bO^{-}=o^{-})}{\Prr(a,o^{-})} \{\Prr(\bO\mid a,\bO^{-} \}^{-1}  d^{\pi^e}(\bO),\quad     d^{\pi^e}(o)=\sum_{k=0}^{\infty}\gamma^k     d^{\pi^e}_k(o)/(1-\gamma) . 
\end{align*}

Now, we are ready to calculate the Cram\'er-Rao lower bound. We have 
\begin{align*}
    \nabla     J(\theta)= B_1 + B_2+B_3
\end{align*}
where 
{\tiny 
\begin{align*}
    B_1 & = \sum_{k=0} \gamma^k \sum_{\mathfrak{j}_{r_k}}r_k \tau_k \nabla  \Prr(r_k, o_k \mid a_k,\bO_{k-1})\{\Prr(\bO_k \mid a_k, \bO_{k-1}\}^{-1}\Prr(\bO_k,o_{k-1}\mid a_k,\bO_{k-2})\{\Prr(\bO_{k-1} \mid a_{k-1}, \bO_{k-2})\}^{-1}\cdots \Prr(\bO_0),\\
    B_2 &= \sum_{\mathfrak{j}}\sum_{k=0} \gamma^k \sum_{t=0}^k r_k\tau_k \Prr(r_k, o_k \mid a_k,\bO_{k-1})\{\Prr(\bO_k \mid a_k, \bO_{k-1}\}^{-1}\cdots  \Prr(\bO_{t+1},o_{t}\mid a_{t},\bO_{t-1})\nabla \{\Prr(\bO_{t} \mid a_{t}, \bO_{t-1})\}^{-1}\cdots \Prr(\bO_0), \\
    B_3 &= \sum_{\mathfrak{j} } \sum_{k=0} \gamma^k \sum_{t=0}^{k-1} r_k\tau_k \Prr(r_k, o_k \mid a_k,\bO_{k-1})\{\Prr(\bO_k \mid a_k, \bO_{k-1}\}^{-1}\cdots  \nabla \Prr(\bO_{t+1},o_{t}\mid a_{t},\bO_{t-1})\{ \Prr(\bO_{t} \mid a_{t}, \bO_{t-1})\}^{-1}\cdots \Prr(\bO_0). 
\end{align*}
}
Here, we use the notation $\mathfrak{j}=\{s_0,a_0,r_0,\cdots \}$. 

We analyze $B_1$:  
{\small 
\begin{align*}
    B_1&=\sum_{k=0} \gamma^k \sum_{\mathfrak{j}_{r_k}}r_k \tau_k \nabla  \Prr(r_k, o_k \mid a_k,\bO_{k-1})\{\Prr(\bO_k \mid a_k, \bO_{k-1}\}^{-1}\Prr(\bO_k,o_{k-1}\mid a_k,\bO_{k-2})\{\Prr(\bO_{k-1} \mid a_{k-1}, \bO_{k-2})\}^{-1}\cdots \Prr(\bO_0)\\
    &=(1-\gamma)^{-1} \sum_{r,a,o } r\epol(a\mid o)\nabla \Prr(r,o\mid a, \bO^{-})\{b_{W}(a,\bO^{-})\odot \Prr(a,\bO^{-}) \} \\  
    &= (1-\gamma)^{-1}\sum_{r,a,o,o^{-} } r\epol(a\mid o)\nabla  \Prr(r,o\mid a, o^{-}) b_{W}(a,o^{-})\Prr(a,o^{-})\\
    &=(1-\gamma)^{-1}\sum_{r,a,o,o^{-} } r\epol(a\mid o)\{\nabla \log \Prr(r,o\mid a, o^{-})\} b_{W}(a,o^{-})\Prr(r,o,a,o^{-}), 
\end{align*}
}
where $\odot$ is an element-wise product. 
Then, we have
\begin{align*}
  (1-\gamma)  B_1  &=  \E[b_{W}(A,O^{-}) R\epol(A\mid O) \nabla \log \Prr(R, O \mid A, O^{-})  ]  \\ 
    &= \E[b_{W}(A,O^{-})\{ R\epol(A\mid O)-\E[ R\epol(A\mid O)\mid A,O^{-}]  \} \nabla \log \Prr(R, O \mid A, O^{-})  ]\\
     &=\E[b_{W}(A,O^{-})\{ R\epol(A\mid O)-\E[ R\epol(A\mid O)\mid A,O^{-}]  \} \nabla \log \Prr(R, O, A, O^{-})  ]\\
         &=  \E[b_{W}(A,O^{-})\{ R\epol(A\mid O)-\E[ R\epol(A\mid O)\mid A,O^{-}]  \} \nabla \log \Prr(O^{+},R, O, A, O^{-})  ].
\end{align*}

Next, we analyze $B_2$: 
{\small 
\begin{align*}
    &\sum_{\mathfrak{j}}\sum_{k=0} \gamma^k \sum_{t=0}^k r_k\tau_k \Prr(r_k, o_k \mid a_k,\bO_{k-1})\{\Prr(\bO_k \mid a_k, \bO_{k-1}\}^{-1}\cdots  \Prr(\bO_{t+1},o_{t}\mid a_{t},\bO_{t-1})\nabla \{\Prr(\bO_{t} \mid a_{t}, \bO_{t-1})\}^{-1}\cdots \Prr(\bO_0) \\ 
    &=\sum_{\mathfrak{j}} \sum_{t=0} \gamma^{t} \sum_{k=t}^{\infty} \gamma^{k-t}\tau_{k} r_k \Prr(r_k, o_k \mid a_k,\bO_{k-1})\{\Prr(\bO_k \mid a_k, \bO_{k-1}\}^{-1}\cdots  \Prr(\bO_{t+1},o_{t}\mid a_{},\bO_{t-1})\nabla \{ \Prr(\bO_{t} \mid a_{t}, \bO_{t-1})\}^{-1}\cdots \Prr(\bO_0) \\ 
   &=\sum_{\mathfrak{j}} \sum_{t=0} \gamma^{t} \sum_{k=t}^{\infty} \gamma^{k-t}\tau_{k} r_k \Prr(r_k, o_k \mid a_k,\bO_{k-1})\{\Prr(\bO_k \mid a_k, \bO_{k-1}\}^{-1}\cdots  \Prr(\bO_{t+1},o_{t}\mid a_{},\bO_{t-1}) \{ \Prr(\bO_{t} \mid a_{t}, \bO_{t-1})\}^{-1}\\
   &\times \{\nabla \Prr(\bO_{t} \mid a_{t}, \bO_{t-1})\}\{ \Prr(\bO_{t} \mid a_{t}, \bO_{t-1})\}^{-1}\cdots \Prr(\bO_0) \\
     &=-\sum_{t=0} \gamma^{t}\tau_t b_{V}(a_t, \bO_t)\{\nabla \Prr(\bO_{t} \mid a_{t}, \bO_{t-1})\}\{ \Prr(\bO_{t} \mid a_{t}, \bO_{t-1})\}^{-1}\cdots \Prr(\bO_0) \\ 
    &=-(1-\gamma)^{-1}\sum_{a} b_{V}(a,\bO)\{\nabla \Prr(\bO\mid a,\bO^{-})\{b_{W}(a,\bO^{-})\odot \Prr(a,\bO^{-}) \}  \}. 
\end{align*}
}
Further, we have 
\begin{align*}
    (1-\gamma)B_2 &= \E[b_{W}(A,O^{-})b_{V}(A,O)\nabla \log \Pr(O\mid A,O^{-}) ] \\ 
     &= \E[b_{W}(A,O^{-})b_{V}(A,O)\{\nabla \log \Pr(O\mid A,O^{-})+ \nabla \log \Pr(R,O^{+} \mid A,O^{-},O)\} ]\\
   &= \E[b_{W}(A,O^{-}) b_{V}(A,O)\nabla \log \Pr(R,O^{+},O \mid A,O^{-}) ] \\
     &= \E[b_{W}(A,O^{-})\{b_{V}(A,O)-\E[b_{V}(A,O)\mid A,O^{-}] \}\nabla \log \Pr(R,O^{+},O \mid A,O^{-}) ] \\ 
     &= \E[b_{W}(A,O^{-})\{b_{V}(A,O)-\E[b_{V}(A,O)\mid A,O^{-}] \}\nabla \log \Pr(R,O^{+},O, A,O^{-}) ]. 
\end{align*}

Finally, we analyze $B_3$: 
{\small 
\begin{align*}
  & \sum_{\mathfrak{j} } \sum_{k=0} \gamma^k \sum_{t=0}^{k-1} r_k\tau_k \Prr(r_k, o_k \mid a_k,\bO_{k-1})\{\Prr(\bO_k \mid a_k, \bO_{k-1}\}^{-1}\cdots  \nabla \Prr(\bO_{t+1},o_{t}\mid a_{t},\bO_{t-1})\{ \Prr(\bO_{t} \mid a_{t}, \bO_{t-1})\}^{-1}\cdots \Prr(\bO_0)\\
 &=\sum_{\mathfrak{j} }  \sum_{t=0} \gamma^{t}\tau_{t} \sum_{k=t+1}^{\infty} \gamma^{k-t}r_k\tau_{t+1:k} \Prr(r_k, o_k \mid a_k,\bO_{k-1})\{\Prr(\bO_k \mid a_k, \bO_{k-1}\}^{-1}\cdots  \nabla \Prr(\bO_{t+1},o_{t}\mid a_{t},\bO_{t-1})\{ \Prr(\bO_{t} \mid a_{t}, \bO_{t-1})\}^{-1}\cdots \Prr(\bO_0)\\
  &=\sum_{\mathfrak{j}}\sum_{t=0} \gamma^{t}\tau_{t}  b_{a_{t+1}}(\bO_{t+1})   \nabla \Prr(\bO_{t+1},o_{t}\mid a_{t},\bO_{t-1})\{ \Prr(\bO_{t} \mid a_{t}, \bO_{t-1})\}^{-1}\cdots \Prr(\bO_0)\\
  &=(1-\gamma)^{-1}\sum_{\mathfrak{j}}\gamma \pi^e(a \mid o)b_{V}(a^{+}, \bO^{+})\nabla \Prr(\bO^{+},o\mid a,\bO^{-})\{b_{W}(A,\bO^{-})\odot \Prr(a,\bO^{-})\}\\
  &=(1-\gamma)^{-1}\sum_{a^+,o^+,o,a,o^{-}}\gamma \pi^e(a \mid o)b_{V}(a^{+}, o^{+})\nabla \log P(o^{+},o\mid a,o^{-})b_{W}(a,o^{-})\Prr(o^{+},o,a,o^{-}). 
\end{align*}
}
Thus, $ (1-\gamma)B_3$ is equal to 
{\small 
\begin{align*}
    &\gamma \E[b_{W}(A,O^{-})\pi^e(A \mid O)\sum_{a^+}b_{V}(a^{+}, O^{+})\nabla \log P(O^{+},O \mid A,O^{-}) ]\\
    &=\gamma \E[b_{W}(A,O^{-})\pi^e(A \mid O)\sum_{a^+}b_{V}(a^{+}, O^{+}) \nabla \log P(R,O^{+},O \mid A,O^{-}) ]\\
   &=\gamma \E[b_{W}(A,O^{-})\{\pi^e(A \mid O)\sum_{a^+}b_{V}(a^{+}, O^{+}) -\E[\pi^e(A \mid O)\sum_{a^+}b_{V}(a^{+}, O^{+}) \mid A,O^{-} ] \} \nabla \log P(R,O^{+},O \mid A,O^{-}) ]\\
     &=\gamma \E[b_{W}(A,O^{-})\{\pi^e(A \mid O)\sum_{a^+}b_{V}(a^{+}, O^{+})- \E[\pi^e(A \mid O)\sum_{a^+}b_{V}(a^{+}, O^{+}) \mid A,O^{-} ] \} \nabla \log P(R,O^{+},O, A,O^{-}) ]. 
\end{align*}
}
Combining all things together, $(1-\gamma)(B_1+B_2+B_3)$ is  
\begin{align*}
    &  \E[b_{W}(A,O^{-})\{ R\epol(A\mid O)-\E[ R\epol(A\mid O)\mid A,O^{-}]  \} \nabla \log \Prr(O^{+},R, O, A, O^{-})  ] \\
    &+\E[b_{W}(A,O^{-})\{b_{V}(A,O)-\E[b_{V}(A,O)\mid A,O^{-}] \}\nabla \log \Pr(R,O^{+},O, A,O^{-}) ]  \\ 
    &+\gamma \E[b_{W}(A,O^{-})\{\pi^e(A \mid O)\sum_{a^+}b_{V}(a^{+}, O^{+})- \E[\pi^e(A \mid O)\sum_{a^+}b_{V}(a^{+}, O^{+}) \mid A,O^{-} ]  \} \nabla \log P(R,O^{+},O, A,O^{-}) ]\\
    &=\E[b_{W}(A,O^{-})\{ R\epol(A\mid O)+\gamma \epol(A\mid O)\sum_{a^+}b_{V}(a^{+}, O^{+}) - b_{V}(A,O)  \}\nabla \log P(R,O^{+},O, A,O^{-})  ]. 
\end{align*}
Hence, the following is $\phi_{\mathrm{EIF}}$: 
\begin{align*}
 \phi_{\mathrm{EIF}}= (1-\gamma)^{-1}b_{W}(A,O^{-})\{ R\epol(A\mid O)+ \gamma \epol(A\mid O)\sum_{a^+}b_{V}(a^{+}, O^{+}) - b_{V}(A,O)  \}. 
\end{align*}
\end{proof}




\begin{proof}[Proof of \pref{thm:efficiency}]

By some algebra, we have 
\begin{align*}
    J(f,g)-  J(b_V,b_W)      =B_1+B_2+B_3 
    %&=\E_{\nu_{\Ocal}}[\sum_{a}g(a,\tilde o)]+f(a,o^-)\{\{R+\gamma \sum_a g(a',O^+)\}\epol(a\mid o)-g(a,o)\} \\
    % &-\{\E_{\nu_{\Ocal}}[\sum_{a}b_V(a,\tilde o)]+b_W(a,o^-)\{\{R+\gamma \sum_a b_W(a',O^+)\}\epol(a\mid o)-b_V(a,o)\}\}\\ 
    % &= \E_{\nu_{\Ocal}}[\sum_{a}g(a,\tilde o)]+f(a,o^-)\{\{\gamma \sum_a \{g(a',O^+)-b_V(a',o^+)\}\}\epol(a\mid o)-g(a,o)+b_V(a',o^+)\} \\
    % &-\{\E_{\nu_{\Ocal}}[\sum_{a}b_V(a,\tilde o)]+\{b_W(a,o^-)-f(a,o^-)\}\{\{R+\gamma \sum_a b_V(a',O^+)\}\epol(a\mid o)-b_V(a,o)\}\}\\ 
 \end{align*}   
 where 
 {\small 
 \begin{align*}
      B_1 &= \{f(a,o^-)-b_W(a,o^-) \}\{\{\gamma \sum_{a'} \{g(a',O^+)-b_V(a',o^+)\}\}\epol(a\mid o)-g(a,o)+b_V(a',o^+)\},  \\
     B_2 &= \E_{\tilde o \sim \nu_{\Ocal}}[\sum_{a'}g(a,\tilde o)]-\E_{\tilde o \sim \nu_{\Ocal}}[\sum_{a'}b_V(a,\tilde o)]+ b_W(a,o^-)\{\gamma \sum_{a'} \{g(a',o^+)-b_V(a',o^+)\}\epol(a\mid o)-g(a,o)+b_V(a,o)\},  \\
    B_3 &= \{b_W(a,o^-)-f(a,o^-)\}\{\{r+\gamma \sum_{a'} b_V(a',o^+)\}\epol(a\mid o)-b_V(a,o)\}\}.
\end{align*}
}
Recall the estimator is constructed as 
\begin{align*}
    \hat J^{*}_{\mathrm{DR}}=0.5 \E_{\Dcal_1}[J(\hat b^{(1)}_W,\hat b^{(1)}_V)]+  0.5 \E_{\Dcal_2}[J(\hat b^{(2)}_W,\hat b^{(2)}_V)]. 
\end{align*}
We analyze $ \E_{\Dcal_1}[J(\hat b^{(1)}_W,\hat b^{(1)}_V)]-J(\epol)$. This is expanded as 
\begin{align*}
    \sqrt{n}(\E_{\Dcal_1}[J(\hat b^{(1)}_W,\hat b^{(1)}_V)]-J(\epol))&=\sqrt{n/n_1}\mathbb{G}_{\mathcal{D}_1} [J(\hat b^{(1)}_W,\hat b^{(1)}_V)-J( b_W,b_V)  ]\\ 
    &+ \sqrt{n/n_1} \mathbb{G}_{\mathcal{D}_1} [J( b_W,b_V) ] \\
    & + \sqrt{n/n_1} (\E[ J( \hat b^{(1)}_W,\hat b^{(1)}_V ) \mid \Dcal_2 ] -J(\epol)  ) 
\end{align*}
where $\mathbb{G}_{\mathcal{D}_1} =\sqrt{n_1}(\E_{\Dcal_1}-\E)$. In the following, we analyze each term.  

\paragraph{Analysis of $\sqrt{n/n_1}\mathbb{G}_{\mathcal{D}_1} [J(\hat b^{(1)}_W,\hat b^{(1)}_V)-J( b_W,b_V)  ]$. }

We show that the conditional variance given $\Dcal_2$ is $o_p(1)$. Then, the rest of the argument is the same as the proof of \cite[Theorem 7]{KallusNathan2019EBtC}. This is proved by 
\begin{align*}
    \mathrm{var}[\sqrt{n_1}\E_{\mathcal{D}_1} [J(\hat b^{(1)}_W,\hat b^{(1)}_V)] \mid \Dcal_2]=\E[B^2_1 + B^2_2 + B^2_3 + 2B_1B_2 + 2B_1B_3 + 2B_1B_2 \mid \Dcal_2 ]=o_p(1). 
\end{align*}
For example, $\E[B^2_3 \mid \Dcal_2]=o_p(1)$ is proved by 
\begin{align*}
    \E[B^2_3 \mid \Dcal_2]\lesssim \E[(\hat b_W-b_W)^2(A,O^-)]\E[\{\Tcal\hat b_V\}^2(A,O^-)]=o_p(1). 
\end{align*}

\paragraph{Analysis of $\sqrt{n/n_1} (\E[ J( \hat b^{(1)}_W,\hat b^{(1)}_V) \mid \Dcal_2  ] -J(\epol)  )$. }

Here,we have
\begin{align*}
&\E[ J( \hat b^{(1)}_W,\hat b^{(1)}_V) \mid \Dcal_2  ]=    |\E[B_1 + B_2 + B_3 \mid \Dcal_2 ]|\\
&= |\E[B_3 \mid \Dcal_2 ]|\leq \E[B^2_3 \mid \Dcal_2 ]^{1/2}\leq \E[(\hat b_W-b_W)^2(A,O^-)]^{1/2}\E[\{\Tcal\hat b_V\}^2(A,O^-)]^{1/2}\\
&=o_p(n^{-1/2}_1) \tag{From convergence rate condition}. 
\end{align*}


\paragraph{Combine all things. }
Thus, 
\begin{align*}
     \sqrt{n}(\E_{\Dcal_1}[J(\hat b^{(1)}_W,\hat b^{(1)}_V)]-J(\epol))=  \sqrt{n/n_1}\mathbb{G}_{\mathcal{D}_1} [J( b_W,b_V) ]+o_p(n^{-1/2}). 
\end{align*}
This immediately concludes 
\begin{align*}
     \sqrt{n}(\hat J^{*}_{DR}-J(\epol))=    \mathbb{G}_n[J( b_W,b_V) ]+o_p(n^{-1/2})
\end{align*}
where $\mathbb{G}_n=\sqrt{n}(\E_{\Dcal}-\E)$. 
\end{proof}


\subsection{Proof of \pref{sec:OPEtimehomo}}

We denote $\E[b'^j_V(A_j,O_i)\mid A_j=a, S_j=s]$  by $Q^j(a,s)$. 

\begin{lemma}\label{lem:help}
 \begin{align*}
      Q^j (A_j,S_j) &=\E[R_j \epol_j(A_j \mid O_j)\mid A_j, {S_j}]+  \gamma\E\bracks{\sum_{a'}Q^{j+1}(a',S_{j+1} )\epol_j(A_j \mid O_j) \mid A_j, {S_j}}. 
 \end{align*}
\end{lemma}

\begin{proof}
From the definition, we have 
\begin{align*}
    Q^j (A_j,S_j) &=\E[R_j \epol_j(A_j \mid O_j )\mid S_j,A_j]+  \E_{\epol}\bracks{\sum_{t=j+1}^{H-1}\gamma^{t-j} R_t\epol_j(A_j\mid O_j)\mid A_j,S_j}. 
 \end{align*}  
Then, 
 \begin{align*}
    &\E_{\epol}\bracks{\sum_{t=j+1} \gamma^{t-j} R_t\epol_j(A_j \mid O_j)\mid A_j,S_j}=\E_{\epol}\bracks{\E_{\epol}\bracks{\sum_{t=j+1}\gamma^{t-j}  R_t \mid  A_j,S_{j+1},O_{j+1},O_j,S_j} \epol_j(A_j \mid O_j)\mid A_j,S_j}\\  
    &= \E\bracks{\sum_{a'}\E_{\epol}[\sum_{t=j+1}\gamma^{t-j} R_t\mid S_{j+1}, A_{j+1}=a',O_{j+1},O_j]\epol_{j+1}(a'\mid {O_{j+1}})\epol_j(A_j\mid O_j)\mid A_j,S_j}\\
&= \E\bracks{\sum_{a'}\E_{\epol}[\sum_{t=j+1}\gamma^{t-j} R_t\mid S_{j+1}, A_{j+1}=a']\epol_{j+1}(a'\mid {O_{j+1}})\epol_j(A_j \mid O_j)\mid A_j,S_j}\\
&= \E\bracks{\sum_{a'}\E_{\epol}[\sum_{t=j+1}\gamma^{t-j} R_t\mid S_{j+1}, A_{j+1}=a']\E[\epol_{j+1}(a'\mid {O_{j+1}})\mid S_{j+1}, A_{j+1}=a'] \epol_j(A_j \mid O_j)\mid A_j,S_j}\\
    % &= \E\bracks{\sum_{a'}\E_{\epol}[\sum_{t=j+1} R_t\epol_{j+1}(a'\mid {O_{j+1}})\epol_j(a\mid O_j)\mid S_{j+1}, A_{j+1}=a',O_{j+1},O_j]\mid A_j=a,S_j}\\
     %&= \E\bracks{\sum_{a'}\E_{\epol}[\sum_{t=j+1} R_t\epol_{j+1}(a'\mid {O_{j+1}})\epol_j(a\mid O_j)\mid S_{j+1}, A_{j+1}=a',O_{j+1},O_j,A_j=a,S_j]\mid A_j=a,S_j}\\
      %   &= \E\bracks{\sum_{a'}\E_{\epol}[\sum_{t=j+1} R_t\epol_{j+1}(a'\mid {O_{j+1}})\epol_j(a\mid O_j)\mid S_{j+1}, A_{j+1}=a',O_{j},A_j=a,S_j]\mid A_j=a,S_j}\\
      %&= \E\bracks{\sum_{a'}\E_{\epol}[\sum_{t=j+1} R_t\epol_{j+1}(a'\mid {O_{j+1}})\mid S_{j+1}, A_{j+1}=a',O_{j}]\epol_j(a\mid O_j)\mid A_j=a,S_j}\\
    %&= \E\bracks{\sum_{a'}\E_{\epol}[\sum_{t=j+1} R_t\mid S_{j+1}, A_{j+1}=a']\epol_{j+1}(a'\mid {O_{j+1}})\epol_j(a\mid O_j)\mid A_j=a,S_j}\\
     %&= \E\bracks{\sum_{a'}\E_{\epol}[\sum_{t=j+1} R_t\epol_{j+1}(a'\mid {O_{j+1}})\mid S_{j+1}, A_{j+1}=a',O_{j+1},O_j]\epol_j(a\mid O_j)\mid A_j=a,S_j}\\
  %&=  \E\bracks{\sum_{a'}\E_{\epol}[\sum_{t=j+1} R_t\mid \ch_{S_{j+1}},A_{j+1}=a']\E[\epol_{j+1}(a'\mid \mathfrak{j}_{O_{j+1}})\mid \ch_{S_{j+1}},A_{j+1}=a']\epol_j(a\mid O_j)\mid A_j=a,\ch_{S_j}=s}\\
    &=  \E\bracks{\sum_{a'}\E_{\epol}[\sum_{t=j+1}\gamma^{t-j} R_t\epol_{j+1}(a'\mid {O_{j+1}})\mid S_{j+1}, A_{j+1}=a']\epol_j(A_j \mid O_j)\mid A_j,S_j}\\
    &= \gamma \E\bracks{\sum_{a'}Q^{j+1}(a', S_{j+1} )\epol_j(A_j \mid O_j)\mid A_j,S_j}. 
\end{align*}

\end{proof}


\begin{lemma}\label{lem:v_recursive_finite}[Learnable reward bridge functions are reward bridge functions]
\begin{align*}
   \E[b'^{[j]}_{V}(A_j,O_{{j}})\mid A_j,\mathfrak{J}_{j-1} ] &=\E[R_j \epol_j(A_j \mid {O_{j}})\mid A_j,\mathfrak{J}_{j-1} ]  +\gamma\E\bracks{\sum_{a'}b^{'[j+1]}_V(a', {O_{j+1}})\epol_j(A_j \mid {O_{j}}) \mid  A_j,\mathfrak{J}_{j-1} }. 
 \end{align*}
\end{lemma}

\begin{proof}
From \pref{lem:help}, we have 
  \begin{align*}
   & \E[b'^{[j]}_{V}(A_j,O_{j})\mid  A_j,S_j] \\
   &=\E[R_j \epol_j(A_j \mid {O_j})\mid  A_j,S_j]+  \gamma\E\bracks{\sum_{a'}\E[b'^{[j+1]}_V(a', {O_{j+1}})| S_{j+1}, O_{j}]\epol_j(A_j \mid {O_j}) \mid  A_j,S_j}\\
    &=\E[R_j \epol_j(A_j \mid {O_j}) \mid  A_j,S_j]+  \gamma\E\bracks{\sum_{a'}b'^{[j+1]}_V(a', {O_{j+1}})\epol_j(A_j \mid {O_j}) \mid  A_j,S_j}. 
 \end{align*}
Then, from $ O_j, O_{j+1}, R_j\perp \mathfrak{J}_{j-1} \mid  A_j,S_j  $, the statement is concluded by 
  \begin{align*}
   \E[\E[b'^{[j]}_{V}(A_j,O_{j})\mid  A_j,S_j]\mid A_j,\mathfrak{J}_{j-1}  ]&= \E[b'^{[j]}_{V}(A_j,{O_j}) \mid A_j,\mathfrak{J}_{j-1}  ], \\
  \E[\E[R_j \epol_j(A_j \mid {O_j}) \mid  A_j,S_j]  \mid A_j,\mathfrak{J}_{j-1}  ]   &=  \E[R_j \epol_j(A_j \mid {O_j})  \mid A_j,\mathfrak{J}_{j-1}  ],  \\ 
  \E\bracks{\E\bracks{\sum_{a'}b'^{[j+1]}_V(a', {O_{j+1}})\epol_j(A_j \mid {O_j}) \mid  A_j,S_j}\mid A_j,\mathfrak{J}_{j-1}  }&=  \E\bracks{\sum_{a'}b'^{[j+1]}_V(a', {O_{j+1}})\epol_j(A_j \mid {O_j}) \mid A_j,\mathfrak{J}_{j-1}}. 
 \end{align*}


 
\end{proof}


\begin{lemma}[Learnable weight bridge functions are weight bridge functions]
\begin{align*}
    \E\bracks{  b'^{[j]}_{W}(A_j,\mathfrak{J}_{j-1} )\epol_j(A_j |O_{j})f(O_{j+1},a')-\rI(A_{j+1}=a') b'^{[j+1]}_{W}(A_{j+1},\mathfrak{J}_{j}) f(O_{j+1},A_{j+1})}=0,\,\forall f:\Ocal\times \Acal \to \RR.  
\end{align*}
and 
\begin{align*}
     \E\bracks{   \sum_{a'} b'^{[j]}_{W}(A_j,\mathfrak{J}_{j-1} )\epol_j(A_j |O_{j})f(O_{j+1},a')- b'^{[j+1]}_{W}(A_{j+1},\mathfrak{J}_{j}) f(O_{j+1},A_{j+1})}=0,\,\forall f:\Ocal\times \Acal \to \RR.  
\end{align*}
\end{lemma}
\begin{proof}
We first prove the first statement: 
\begin{align*}
     &  \E\bracks{  b'^{[j]}_{W}(A_j,\mathfrak{J}_{j-1} )\epol_j(A_j |O_{j})f({O_{j+1}},a')-\rI(A_{j+1}=a') b'^{[j+1]}_{W}(A_{j+1},\mathfrak{J}_j) f({O_{j+1}},A_{j+1})}\\
    &= \E\bracks{ \E[ b'^{[j]}_{W}(A_j,\mathfrak{J}_{j-1} )\mid A_j, O_j ,S_j,O_{j+1}]\epol_j(A_j |O_{j})f({O_{j+1}},a')} \\ &-\E\bracks{\rI(A_{j+1}=a') \E[b'^{[j+1]}_{W}(A_{j+1},\mathfrak{J}_j) \mid O_{j+1},A_{j+1},S_{j+1}] f({O_{j+1}},A_{j+1})}\\
     &=\E\bracks{  \mu(S_j)\eta_j(A_j|O_{j})f({O_{j+1}},a')- \rI(A_{j+1}=a') \frac{ \mu(S_{j+1})}{P_{\pi_b}(A_{j+1}\mid S_{j+1})}f({O_{j+1}},A_{j+1})}\\
     &=\E_{\epol}[f(O_{j+1},a')]-\E_{\epol}[f(O_{j+1},a')]\\ 
     &=0. 
\end{align*}
Then, we can prove the second statement by taking summation over the action space. 

\end{proof}

\begin{lemma}[Identification formula with unlearnable bridge functions] \label{lem:fake_finite}

Assume the existence of bridge functions. Then, let $b'_V=\{b'^{[j]}_{V}\},b'_W=\{b'^{[j]}_{W}\}$ be any bridge functions. 
\begin{align*}
    J(\epol)=\E\bracks{\sum_j \gamma^j b'^{[j]}_{W}(A_j,\mathfrak{J}_{j-1} )\epol_j(A_j\mid O_j) R_j },\quad J(\epol)=\E\bracks{\sum_a b'^{[0]}_{V}(a,O_0)  }.
\end{align*}

\end{lemma}

\begin{proof}
We prove the first formula:  
\begin{align*}
 \E\bracks{\sum_j \gamma^j b'^{[j]}_{W}(A_j,\mathfrak{J}_{j-1} )\epol_j(A_j\mid O_j) R_j }       &= \E\bracks{\sum_j \gamma^j \E[b'^{[j]}_{W}(A_j,\mathfrak{J}_{j-1} )\mid A_j,S_j]\epol_j(A_j\mid O_j) R_j } \\ 
         &= \E\bracks{\sum_j \gamma^j\frac{\mu_j(S_j)}{P_{\pi_b}(A_j \mid S_j)}\epol_j(A_j\mid O_j) R_j } \tag{Definition of bridge functions}\\
         &=    J(\epol) .  
\end{align*}

We prove the second formula: 
\begin{align*}
      &  \E\bracks{\sum_a b'^{[0]}_{V}(a,O_0)  }= \E\bracks{\E[\sum_a b'^{[0]}_{V}(a,O_0)\mid S_0]  }= \E\bracks{\E[\sum_a b'^{[0]}_{V}(a,O_0)\mid S_0,A_0=a]  }\\
      &= \E\bracks{\sum_a\E_{\epol}[\sum_{t=0}^{H-1} \gamma^{t}R_t  \epol_0(a\mid O_0) \mid S_0,A_0=a]  } \tag{Definition of bridge functions}\\ 
      &= \E\bracks{\sum_a\E_{\epol}[\sum_{t=0}^{H-1} \gamma^{t}R_t  \mid S_0,A_0=a]\E[\epol_0(a\mid O_0)\mid S_0,A_0=a ] }\\
      &= \E\bracks{\sum_a\E_{\epol}[\sum_{t=0}^{H-1} \gamma^{t}R_t  \mid S_0,A_0=a] \epol_0(a\mid O_0) } \\ &=J(\epol).  
\end{align*}

\end{proof}


\begin{lemma}[Final identification formula] \label{thm:finite_identi}
~
\begin{itemize}
    \item Assume the existence of bridge functions. Let  $b_V=\{b^{[j]}_{V}\},b_W=\{b^{[j]}_W\}$ be any learnable bridge functions. 

\begin{align*}
    J(\epol)= \E[\sum_a b^{[0]}_{V}(a,O_0) ], \quad    J(\epol)=\E\bracks{\sum_{j=0}^{H-1} \gamma^j b^{[j]}_{W}(A_j,\mathfrak{J}_{j-1} )\epol_j(A_j\mid O_j) R_j }  . 
\end{align*}
    \item Assume the existence of learnable value bridge functions and the completeness:
    \begin{align*}
        \EE[g(S_j,A_j) \mid A_j,\mathfrak{J}_{j-1}  ]=0 \implies g(\cdot)=0.
    \end{align*}
    Then, 
    \begin{align*}
    J(\epol)= \E[\sum_a b^{[0]}_{V}(a,O_0) ]  . 
\end{align*}
\end{itemize}



\end{lemma}

\begin{proof}
We provide the proof without completeness. The proof with completeness is given in \pref{thm:identimein_non_reactiv}. We prove the first formula: 
\begin{align*}
J(\epol) &= \E\bracks{\sum_j \gamma^j b'^{[j]}_{W}(A_j,\mathfrak{J}_{j-1} )\epol_j(A_j\mid O_j) R_j } \tag{From \pref{lem:fake_finite}}\\ 
    &= \E\bracks{\sum_j \gamma^j b'^{[j]}_{W}(A_j,\mathfrak{J}_{j-1} )\E[\epol_j(A_j\mid O_j) R_j \mid A_j, \mathfrak{J}_{j-1} ] } \\
    &= \E\bracks{\sum_j \gamma^j b'^{[j]}_{W}(A_j,\mathfrak{J}_{j-1} )\{\gamma \sum_a \E[b^{[j+1]}_V(a,O_{j+1})\epol_j(A_j \mid O_j)  \mid A_j, \mathfrak{J}_{j-1}  ]-\E[b^{[j]}_{V}(A_j,O_j)  \mid A_j, \mathfrak{J}_{j-1}  ]  \} } \tag{$b_V$ are value bridge functions.}\\
    &=  \sum_{j=1}^{H-1} \gamma^j \E\bracks{ b'^{j-1}_W(A_{j-1},{\mathfrak{J}_{j-2}})\epol_{j-1}(A_{j-1} \mid O_{j-1})\sum_a  b^{[j]}_V(a,O_{j}) -  b'^{[j]}_{W}(A_j,\mathfrak{J}_{j-1} ) b^{[j]}_{V}(A_j,O_j)   }\\
    &+\E[\sum_a b^{[0]}_{V}(a,O_0) ] \\
    &= \E[\sum_a b^{[0]}_{V}(a,O_0) ]. \tag{Value bridge functions are learnable bridge functions.  }  
\end{align*}
Next, we prove the second formula: 
\begin{align*}
    J(\epol)&= \E[\sum_a b'^{[0]}_{V}(a,O_0) ] \tag{From \pref{lem:fake_finite}}\\ 
        &= \sum_{j=1}^{H-1} \gamma^j \E\bracks{ b^{[j-1]}_W(A_{j-1},\mathfrak{J}_{j-2})\epol_{j-1}(A_{j-1} \mid O_{j-1})\sum_a  b'^{[j]}_V(a,O_{j}) -  b^{[j]}_{W}(A_j,\mathfrak{J}_{j-1} ) b'^{[j]}_V(A_j,O_j)   } \tag{Definition of weight bridge functions}\\
    &+\E[\sum_a b'^{[0]}_{V}(a,O_0) ]\\
&= \E\bracks{\sum_j \gamma^j b^{[j]}_{W}(A_j,\mathfrak{J}_{j-1} )\{\gamma \sum_a \E[b'^{(j+1)}_V(a,O_{j+1})\epol_j(A_j \mid O_j)  \mid A_j, \mathfrak{J}_{j-1}  ]-\E[b'^j_V(A_j,O_j)  \mid A_j, \mathfrak{J}_{j-1}  ]  \} }\\
  &= \E\bracks{\sum_j \gamma^j b^{[j]}_{W}(A_j,\mathfrak{J}_{j-1} )\E[\epol_j(A_j\mid O_j) R_j \mid A_j, \mathfrak{J}_{j-1} ] } \tag{Reward bridge functions are learnable reward bridge functions}\\
  &=\E\bracks{\sum_j \gamma^j b^{[j]}_{W}(A_j,\mathfrak{J}_{j-1} )\epol_j(A_j\mid O_j) R_j }.  
\end{align*}
\end{proof}



\begin{proof}[Proof of \pref{lem:nair}]
This is proved in \citet[Theorem 3]{nair2021spectral}.  Especially, our formula is their specific formula when using left singular vectors for $M$. We refer the readers to read their proof. 
\end{proof}

Next, we prove the doubly robust property. 

\begin{proof}[Proof of \pref{thm:doubly_finite}]
The first statement $J(\epol)=\E[J(b_V,g)]$ is proved by the definition of reward bridge functions: 
\begin{align*}
  &\E\bracks{\sum_a  b^{[0]}_V(a,O_0)+\sum_{k=0}^{H-1}\gamma^k  g^{[k]}(A_k,\mathfrak{J}_{k-1})\prns{\epol_k(A_k \mid O_k)\{R_k+\gamma \sum_{a^+} b^{[k+1]}_V(a^+,O_{k+1}) \}-  b^{[k]}_V(A_k,O_k) }}\\
  &=   \E\bracks{\sum_a  b^{[0]}_V(a,O_0)+\sum_{k=0}^{H-1}\gamma^k \hat g^{[k]}(A_k,\mathfrak{J}_{k-1})\E\prns{\epol_k(A_k \mid O_k)\{R_k+\gamma \sum_{a^+}\hat b^{[k+1]}_V(a^+,O_{k+1}) \}-  b^{[k]}_V(A_k,O_k)\mid A_k,\mathfrak{J}_{k-1} }}\\
  & = \E\bracks{\sum_a  b^{[0]}_V(a,O_0)}  \tag{From the definition of  reward bridge functions}\\
  &= J(\epol) \tag{From identification results, \pref{thm:finite_identi}}. 
\end{align*}
The second statement $J(\epol)=\E[J(f,b_W)]$ is proved by the definition of weight bridge functions:
\begin{align*}
     & \E\bracks{\sum_a f^{[0]}(a,O_0)+\sum_{k=0}^{H-1}\gamma^k  b^{[k]}_W(A_k,\mathfrak{J}_{k-1})\prns{\epol_k(A_k \mid O_k)\{R_k+\gamma \sum_{a^+}f^{[k+1]}(a^+,O_{k+1}) \}- f^{[k]}(A_k,O_k) }}\\
    &= \E\bracks{\sum_{k=0}^{H-1}\gamma^k  b^{[k]}_W(A_k,\mathfrak{J}_{k-1})\epol_k(A_k \mid O_k)R_k }+ \\
    &+\E\prns{\sum_{k=1}^{H-1}\gamma^k  b^{[k-1]}_W(A_{k-1},\mathfrak{J}_{k-2})\epol_{k-1}(A_{k-1} \mid O_{k-1}) \sum_{a^+}f^{[k]}(a^+,O_{k})-\gamma^k b^{[k]}_W(A_k,\mathfrak{J}_{k-1}) f^{[k]}(A_k,O_k) }\\
    &= \E\bracks{\sum_{k=0}^{H-1}\gamma^k  b^{[k]}_W(A_k,\mathfrak{J}_{k-1})\epol_k(A_k \mid O_k)R_k } \tag{From the definition of  weight bridge functions}\\
      &= J(\epol) \tag{From identification results, \pref{thm:finite_identi}}.  
\end{align*}




\end{proof}





\begin{proof}[Prof of \pref{thm:identimein_non_reactiv}]

~
\paragraph{With Completeness }
From the definition of bridge functions: 
\begin{align*}
    \E\bracks{\epol_j(A_j\mid O_j,\mathfrak{\tilde J}_{j-1}) R_j +\sum_a \gamma b^{[j+1]}_V(a,O_{j+1},\mathfrak{\tilde J}_{j} )\epol_j(A_j \mid O_j,\mathfrak{\tilde J}_{j-1} ) - b^{[j]}_V(A_j,O_{j},\mathfrak{\tilde J}_{j-1} )\mid A_j,\mathfrak{J}_{j-1} }= 0. 
\end{align*}
Using the completeness, we have 
\begin{align*}
    \E\bracks{\epol_j(A_j\mid O_j,\mathfrak{\tilde J}_{j-1}) R_j +\sum_a \gamma b^{[j+1]}_V(a,O_{j+1},\mathfrak{\tilde J}_{j} )\epol_j(A_j \mid O_j,\mathfrak{\tilde J}_{j-1} ) - b^{[j]}_V(A_j,O_{j},\mathfrak{\tilde J}_{j-1} ) \mid  S_j,A_j,\mathfrak{\tilde J}_{j-1} }= 0. 
\end{align*}

Now, we are ready to prove the main statement. 
We denote $ \mu_{j}(S_j, \mathfrak{\tilde J}_{j-1}) =\EE[\prod_{k=0}^{j-1} \frac{\epol_k(A_k\mid O_k,\mathfrak{J}_{k-1}) }{\pi_b(A_k \mid S_k) } \mid S_j,\mathfrak{\tilde J}_{j-1} ]  $.  Then, we have 
{\small 
\begin{align*}
&J(\epol)= \E\bracks{\sum_j \gamma^j  \frac{\mu_{j}(S_j, \mathfrak{\tilde J}_{j-1})}{\pi_b(A_j \mid S_j)} \epol_j(A_j\mid O_j,\mathfrak{\tilde J}_{j-1}) R_j } \\ 
    &= \E\bracks{\sum_j \gamma^j  \frac{\mu_{j}(S_j, \mathfrak{\tilde J}_{j-1})}{\pi_b(A_j \mid S_j)} \E\bracks{\epol_j(A_j\mid O_j,\mathfrak{\tilde J}_{j-1}) R_j \mid S_i,A_j,\mathfrak{\tilde J}_{j-1} } } \\
    &= \E\bracks{\sum_j \gamma^j \frac{\mu_{j}(S_j, \mathfrak{\tilde J}_{j-1})}{\pi_b(A_j \mid S_j)}\{\gamma \sum_a \E[b^{[j+1]}_V(a,O_{j+1},\mathfrak{\tilde J}_{j} )\epol_j(A_j \mid O_j,\mathfrak{\tilde J}_{j} )  \mid S_j, A_j, \mathfrak{\tilde J}_{j-1}  ]-\E[b^{[j]}_{V}(A_j,O_j,\mathfrak{\tilde J}_{j-1} )  \mid S_j,A_j, \mathfrak{\tilde J}_{j-1}  ]  \} }  \\
    &=  \sum_{j=1}^{H-1} \gamma^j \E\bracks{  \frac{\mu_{j-1}(S_{j-1}, \mathfrak{\tilde J}_{j-2})}{\pi_b(A_{j-1} \mid S_{j-1})} \epol_{j-1}(A_{j-1} \mid O_{j-2},\mathfrak{\tilde J}_{j-2} )\sum_a  b^{[j]}_V(a,O_{j},\mathfrak{\tilde J}_{j-1} ) -  \frac{\mu_{j}(S_j, \mathfrak{\tilde J}_{j-1})}{\pi_b(A_j \mid S_j)} b^{[j]}_{V}(A_j,O_j,\mathfrak{\tilde J}_{j-1} )   }\\
    &+\E[\sum_a b^{[0]}_{V}(a,O_0) ]= \E[\sum_a b^{[0]}_{V}(a,O_0) ].  
\end{align*}
}

\paragraph{Without Completeness }

From the definition of bridge functions: 
\begin{align*}
    \E\bracks{\epol_j(A_j\mid O_j,\mathfrak{\tilde J}_{j-1}) R_j +\sum_a \gamma b^{[j+1]}_V(a,O_{j+1},\mathfrak{\tilde J}_{j} )\epol_j(A_j \mid O_j,\mathfrak{\tilde J}_{j-1} ) - b^{[j]}_V(A_j,O_{j},\mathfrak{\tilde J}_{j-1} )\mid A_j,\mathfrak{\tilde J}_{j-1} }= 0. 
\end{align*}


Now, we are ready to prove the main statement. 
We denote $ \mu_{j-1}(S_j, \mathfrak{\tilde J}_{j-1}) =\EE[\prod_{k=0}^{j-1} \frac{\epol_k(A_k\mid O_k, \mathfrak{\tilde J}_{k-1}) }{\pi_b(A_k \mid S_k) } \mid S_j,A_j,\mathfrak{J}_{j-1} ]  $.  Then, we have 
{\small 
\begin{align*}
&J(\epol)= \E\bracks{\sum_j \gamma^j  \frac{\mu_{j}(S_j, \mathfrak{\tilde J}_{j-1})}{\pi_b(A_j \mid S_j)} \epol_j(A_j\mid O_j, \mathfrak{\tilde J}_{j-1}) R_j } \\ 
  &=  \E\bracks{\sum_j \gamma^j  \braces{\EE[ b^{[j]}_W(A_j,\mathfrak{J}_{j-1}) \mid   S_j,A_j, \mathfrak{\tilde J}_{j-1}] }  \epol_j(A_j\mid O_j,\mathfrak{\tilde J}_{j-1}) R_j }  \\ 
    &= \E\bracks{\sum_j \gamma^j  b^{[j]}_W(A_j,\mathfrak{J}_{j-1}) \epol_j(A_j\mid O_j,\mathfrak{\tilde J}_{j-1}) R_j  } \\
   %%% &= \E\bracks{\sum_j \gamma^j  \frac{b^{[j]}_W(\cj_{j-1})}{\pi_b(A_j \mid S_j)} \epol_j(A_j\mid O_j,\mathfrak{\tilde J}_{j-1}) R_j  } \\
    &= \E\bracks{\sum_j \gamma^j   b^{[j]}_W(A_j, \mathfrak{J}_{j-1})\{\gamma \sum_a \E[b^{[j+1]}_V(a,O_{j+1},\mathfrak{\tilde J}_{j} )\epol_j(A_j \mid O_j, \mathfrak{\tilde J}_{j-1} )   - b^{[j]}_{V}(A_j,O_j, \mathfrak{\tilde J}_{j-1} )  \mid A_j, \mathfrak{J}_{j-1}  ]  \} }  \\
      &= \E\bracks{\sum_j \gamma^j  \frac{\mu_{j}(S_{j}, \mathfrak{\tilde J}_{j-1})}{\pi_b(A_{j} \mid S_{j})}   \{\gamma \sum_a \E[b^{[j+1]}_V(a,O_{j+1},\mathfrak{\tilde J}_{j} )\epol_j(A_j \mid O_j, \mathfrak{\tilde J}_{j-1} )   - b^{[j]}_{V}(A_j,O_j, \mathfrak{\tilde J}_{j-1} )  \mid A_j,\mathfrak{J}_{j-1}  ]  \} }  \\
    &=  \sum_{j=1}^{H-1} \gamma^j \E\bracks{  \frac{\mu_{j-1}(S_{j-1}, \mathfrak{\tilde J}_{j-2})}{\pi_b(A_{j-1} \mid S_{j-1})} \epol_{j-1}(A_{j-1} \mid O_{j-1},\mathfrak{\tilde J}_{j-1} )\sum_a  b^{[j]}_V(a,O_{j},\mathfrak{\tilde J}_{j-1} ) -  \frac{\mu_{j}(S_j, \mathfrak{\tilde J}_{j-1})}{\pi_b(A_j \mid S_j)} b^{[j]}_{V}(A_j,O_j,\mathfrak{\tilde J}_{j-1} )   }\\
    &+\E[\sum_a b^{[0]}_{V}(a,O_0) ]= \E[\sum_a b^{[0]}_{V}(a,O_0) ].  
\end{align*}
}
\end{proof}


\subsection{Proof of \pref{app:morePOMDP}}



\begin{proof}[Proof of \pref{thm:without}]
From Hoeffding inequality, we use with probability $1-\delta$: 
\begin{align*}
  \forall f\in \Vcal, \forall g\in \Vcal^{\dagger}; | (\E-\E_{\Dcal})\bracks{f(A,O^{-})\Zcal g(A,O^{-})  }|\leq c \{\max(1,C_{\Vcal},C_{\Vcal^{\dagger}}) \}\sqrt{\log(|\Vcal||\Vcal^{\dagger}|/\delta)/n}. 
\end{align*}
Recall $\Zcal f=R\epol(a\mid o)+\sum_{a'} f(a',O^+)\epol(a\mid o)$. Hereafter, we condition this event.

In this proof, we often use the following:
\begin{align*}
    \E[f(A,O^{-})\Zcal g(A,O^{-})] =   \E[f(A,O^{-})\Tcal g(A,O^{-})]. 
\end{align*}
Recall $\Tcal g=\E[R\epol(A\mid O)+\sum_{a'} f(a',O^+)\epol(a\mid O)\mid A=a,O^-=o] $. 

As a first step, we have 
\begin{align*}
    |J(\epol)- \hat J_{\VM}|&\leq \left|(1-\gamma)^{-1}\E\bracks{b_W(A,O^{-})\Tcal \hat b_V(A,O^{-}) }\right|. 
\end{align*}
Then,
\begin{align*}
    \left|\E\bracks{b_W(A,O^{-})\Tcal \hat b_V(A,O^{-})}\right|
    &\leq \left|(\E-\E_{\Dcal})\bracks{b_W(A,O^{-})\Zcal \hat b_V(A,O^-)}\right| + \left|\E_{\Dcal}\bracks{b_W(A,O^{-})\Zcal \hat b_V(A,O^{-})}\right| \\ 
    &\leq c\sqrt{\log(|\Vcal||\Vcal^{\dagger}|c/\delta)/n}+\sup_{f\in \Vcal^{\dagger}}\left|\E_{\Dcal}\bracks{f(A,O^{-})\Zcal \hat b_V(A,O^{-})}\right|  \tag{$b_W\in \Vcal^{\dagger}$} \\ 
    &\leq c\sqrt{\log(|\Vcal||\Vcal^{\dagger}|c/\delta)/n}+\sup_{f\in \Vcal^{\dagger}}\left|\E_{\Dcal}\bracks{f(A,O^{-})\Zcal b_V(A,O^{-})}\right| \tag{$b_V\in \Vcal$} \\ 
     &\leq 2c\sqrt{\log(|\Vcal||\Vcal^{\dagger}|c/\delta)/n}. 
\end{align*}
In the final line,  we use 
\begin{align*}
    \E\bracks{f(A,O^{-})\Tcal b_V(A,O^{-})}=0,\quad \forall f:\Acal\times \Ocal \to \RR; 
\end{align*}
thus, 
\begin{align*}
     & \sup_{f\in \Vcal^{\dagger}}\left|\E_{\Dcal}\bracks{f(A,O^{-})\Zcal b_V(A,O^{-})}\right|\\
    &=\left|\E_{\Dcal}\bracks{f^{\diamond}(A,O^{-})\Zcal b_V(A,O^{-})}\right| \tag{ $f^{\diamond}=\max_{f\in \Vcal^{\dagger}}\left|\E_{\Dcal}\bracks{f(A,O^{-})\Zcal b_V(A,O^{-})}\right|$ } \\
    &\leq \left|\E[\bracks{f^{\diamond}(A,O^{-})\Zcal b_V(A,O^{-})}\right| + c\sqrt{\log(|\Vcal||\Vcal^{\dagger}|c/\delta)/n} \\
    &=  \left|\E[\bracks{f^{\diamond}(A,O^{-})\Tcal b_V(A,O^{-})}\right| + c\sqrt{\log(|\Vcal||\Vcal^{\dagger}|c/\delta)/n}= c\sqrt{\log(|\Vcal||\Vcal^{\dagger}|c/\delta)/n}. 
\end{align*}


\end{proof}





==> time_homogeneous.tex <==
\section{OPE in Time-homogeneous POMDPs}\label{sec:OPEtimehomo} 

%Before considering OPE of time-imhomogeneous POMDPs, for the simplicity of notation, 
In this section, we focus on time-homogeneous POMDPs where $P_t,Z_t,r_t,\epol_t,\bpol_t$ are stationary over time. We denote them by $P,Z,r,\epol,\bpol$, respectively. The goal is to estimate the target policy's value in infinite-horizon settings where $H=+\infty$ and $J(\pi)=\E_{\pi}[\sum_{t=0}^{+\infty}\gamma^t R_t]$. 
%We suppose we have $n$ i.i.d transitions $\Dcal$ consisting of $\{O^{-},O,A,R,O^{+}\}$  following 
%Consider a data tuple $(S^-,O^{-},A^-,S,O,A,R,S^+,O^{+})$ from $\{(S_{t-1},O_{t-1},A_{t-1},S_t,O_t,A_t,R_t,S_{t+1},O_{t+1}):t\ge 1\}$. Under the POMDP model assumption, we have
%\begin{align*}
%    O^{-}\sim Z(\cdot|S^{-}), A^{-}\sim \pi_b(\cdot|S^{-}), S\sim P(\cdot|S^-,A^-), O\sim Z(\cdot|S), A\sim \bpol(\cdot|S),S^+ \sim P(\cdot|S,A),\\R=r(S,A,S^+),O^{+}\sim Z(\cdot|S^+). 
%\end{align*}
%\begin{align*}
%   S^{-}\sim P_{\bpol}(\cdot), O^{-}\sim Z(\cdot|S^{-}), S\sim \sum_a P(\cdot|S^-,a)\pi_b(a\mid S^-), O\sim Z(\cdot|S), A\sim \bpol(\cdot|S),S^+ \sim P(\cdot|S,A),\\R=r(S,A,S^+),O^{+}\sim Z(\cdot|S^+), 
%\end{align*} 
Consider a data tuple $(O^{-},S,O,A,R,S^+,O^{+})$ following 
%\masa{I still suggest following. Since this is the most general data configuraiton and clean. I showed the conversion as one example. }
\begin{align*}
   (O^-,S) \sim P_{\bpol}(\cdot), A\sim \bpol(\cdot|S),S^+ \sim P(\cdot|S,A),R=r(S,A),O^{+}\sim Z(\cdot|S^+), 
\end{align*}
where $P_{\bpol}(\cdot)$ denotes certain distribution over $\Ocal\times \Scal$. For example, the data $\{O_{t-1},S_t,O_t,A_t,R_t,S_{t+1},O_{t+1}):t\ge 1\}$ satisfies this configuration. 
We assume the initial observation distribution $\nu_{\Ocal}(o)\coloneqq \int Z(o\mid s)\nu(s)\rd(s)$ is known to us. %\footnote{If it is unknown, we need to estimate from the data and plug-in.}. 
If unknown, it can be estimated by the empirical data distribution.
%Recall we \emph{cannot} observe $S^-$, $S$ and $S^+$. 
With a slight abuse of notation, we denote the distribution of the %observed 
data as $P_{\bpol}(\cdot)$, e.g., $P_{\bpol}(a\mid s)=\bpol(a\mid s)$. 
%{\color{blue}Let $d_{\epol}(s)$ be a discounted occupancy measure w.r.t $\epol$ and the same POMDP.} %The corresponding Bayesian network is illustrated in \pref{fig:POMDP_homo}. 

%In this section, 
The rest of this section is organized as follows. We first present the identification method for the target policy's value. We next introduce the proposed value estimator. Finally, we study their nonasymptotic and asymptotic properties. 
%Then, we introduce estimation methods by formulating bridge functions into estimation equations and leveraging minimax estimation. Next, we show their finite and asymptotic guarantees. Finally, we provide the Cram\'er-Rao lower bound of the policy value in the tabular setting. 

\subsection{Identification}\label{subsec:identify_homo}

%We discuss the identification way. First of all, we define bridge functions. 
First, we extend our definitions of the bridge functions to the POMDP setting and require their existence in the assumption below. Let $w(s)=\sum_{t\ge 0} \gamma^t P_{\epol,t}(s)/P_{\bpol}(s)$ denote the marginal density ratio where $P_{\epol,t}(\cdot)$ denotes the probability density function of $S_t$ under the evaluation policy.  %\masa{I removed $\infty$ because i don't want to give the impression the existence of stationary distribution is needed. }
%and $P_{\bpol,\infty}$ denotes the stationary distribution of the state under the behavior policy. 
In addition, let $q^{\epol}(a,s)= \E_{\epol} [\sum_{t\ge 0}\gamma^t R_t|A_0=a,S_0=s]$ denote the Q-function. These functions play an important role in constructing marginal IS and value function-based estimators in fully observable MDPs. The following bridge functions play similar roles in POMDPs. 
%OPE with fully observed state variables. 

\begin{assum}[Existence of bridge functions]\label{assum:existence}
There exist value bridge functions $b'_V:\Acal\times \Ocal\to \RR$ and weight bridge functions $b'_W:\Acal\times \Ocal\to \RR $ that satisfy $\forall (s,a)\in \{(s,a)\in \Scal \times \Acal: \frac{ w(s)\E[\epol(a\mid o)\mid s]}{P_{\bpol}(a|s)}>0\}$: 
\begin{align*}
    \E[b'_{V}(A_0,O_0)\mid A_0=a,S_0=s] &=\E_{\epol}[\sum_t \gamma^t R_t\epol(A_0 \mid O_0)|A_0=a,S_0=s], \\
    \E[b'_{W}(A,O^{-}) \mid A=a,S=s]  &= \frac{ w(s)}{P_{\bpol}(a|s)}.
\end{align*}
%where $w(s)=d_{\epol}(s)/P_{\bpol}(s)$. 
\end{assum}

We make several remarks. First, the existence of $b'_W$ implicitly requires the overlap condition, i.e., for any $s$, $P_{\bpol}(s)=0 \Rightarrow \sum_{t\ge 0} \gamma^t p_t^{\epol}(s)=0$. Second, when the states are fully observed and $\Scal=\Ocal$, it follows immediately that 
%the functions 
%$b_W(\cdot)$ serves as like the marginal weight of an MDP and $b_V(\cdot)$ serves as the Q-function of an MDP. In MDPs ($\Scal=\Ocal$), 
$b'_V(a,s)=q^{\epol}(a,s)\epol(a\mid s)$ and $b'_W(a,s)=w(s)/\bpol(a\mid s)$. Similar to the bandit setting, these bridge functions can thus be interpreted as projections of the value functions and the marginaal IS weights onto the the observation space. Third, we do not require the bridge functions to be uniquely defined. 
%where $q^{\epol}$ is a q-function under $\epol$. 

%Again, we stress out we do not require the uniqueness of solutions. 

Next, we define the learnable bridge functions. 

\begin{definition}[Learnable bridge functions]
Learnable value bridge functions $b_V:\Acal\times \Ocal\to \RR$ are defined as solutions to 
\begin{align}\label{eqn:observed_value}
   \E[b_{V}(A,O)\mid A,O^{-}] &=\E[R \epol(A\mid O)\mid A,O^{-}]+  \gamma\E\bracks{\sum_{a'}b_{V}(a',O^{+})\epol(A \mid O) \mid  A,O^{-}}. 
 \end{align}
Learnable weight bridge functions $b_W:\Acal\times \Ocal \to \RR$ are defined as solutions to 
\begin{align}\label{eq:observed_reward}
\E[L_{\mathbb{W}}(b_W,f)  ]=0,\quad \forall f:\Ocal\times \Acal \to \RR
\end{align}
where 
\begin{align*}
 L_{\mathbb{W}}(g,f)=\E\bracks{\sum_{a'}\gamma  g(A,O^{-})\epol(A|O)f(O^{+},a')-g(A,O^{-}) f(O,A) }+(1-\gamma)\E_{\tilde O\sim \nu_{\Ocal}}[\sum_{a'}f(\tilde O,a')]=0.
\end{align*}
\end{definition}

These definitions are %reduced to the ones in
consistent with those in \pref{def:observed_bridge_bandit} when $\gamma=0$. %Similar to the bandit setting, any bridge function is a learnable bridge function, but the reverse is not true. 

Finally, we show our key identification formula under Assumption \ref{assum:existence}. It extends \pref{lem:observed} and \pref{thm:final_step} to the POMDP setting.

%\masa{i changed the statement way}
\begin{theorem}[Key identification theorem]\label{thm:key_rl} 
%Suppose Assumption \ref{assum:existence} holds.  
~
\begin{enumerate}
    \item Any bridge function is a learnable bridge function. 
    \item Suppose the existence of the value bridge function and learnable weight bridge function $b_W(\cdot)$. Then,  $$ J(\epol)=\frac{1}{1-\gamma} \E[b_{W}(A, O^{-})R\pi(A\mid O)].$$ 
    \item Suppose the existence of the weight bridge function and learnable value bridge function $b_V(\cdot)$. Then, $$J(\epol)=\E_{\tilde O\sim \nu_{\Ocal}}[\sum_a b_V(a,\tilde O)] .$$
\end{enumerate}
\end{theorem}
Similar to the bandit setting, any bridge function is a learnable bridge function, but the reverse is not true. However, the target policy's value can be consistently estimated based on any learnable bridge function. Theorem \ref{thm:key_rl} forms the basis of our estimating procedure. It outlines a marginal IS estimator and a value function-based estimator for policy evaluation.  We remark that assumptions in bullet points 2 and 3 do not imply each other. In addition, when Assumption \pref{assum:existence} holds, %implies 
the assumption in 2 and 3 are automatically satisfied.%from the statement (1). 
%\masa{ i changed here. }

%Given observed bridge functions, this theorem provides the two formulae for the identification: marginal IS way and value-based way. Both formulae are fundamentally different. 
%In the proof, we show Assumption \ref{assum:existence} can be further relaxed depending on the estimator we use.  \masa{i changed here. Do you think we should state in the statemet if this is cofuding? }
%In other words, consistency of the marginal IS estimator requires the existence of the value bridge function and learnable weight  bridge function. Value-based estimator requires the existence of the weight bridge function and learnable value bridge function. 
%In other words, consistency of the marginal IS (or value-based) estimator requires the existence of the learnable weight (or value) bridge function only. 
% whereas consistency of the value-based estimator requires the existence of the value bridge function. 
%formula holds under the existence of observed weight bridge function and (unobserved) reward bridge functions, and the value-based formula holds under the existence of observed reward bridge functions and (unobserved) weight bridge functions. 


\subsection{Estimation}\label{subsec:estimation}

%We discuss the estimation strategy. 
We propose three value estimators given certain consistently estimated learnable bridge functions $\hat b_V$ and $\hat b_W$. %for $b_V$ and $b_W$. Then, we turn to the estimation ways for $b_V$ and $b_W$.  
After that, we will introduce minimax estimation methods for $b_V$ and $b_W$. 

Given some $\hat b_V$ and $\hat b_W$, we can construct the following IS and value function-based estimators accordingly to 
%from 
\pref{thm:key_rl}. Specifically, define %the policy value estimators are naturally introduced: 
\begin{align*}
    \hat J_{\IS}=\frac{1}{1-\gamma}\E_{\Dcal}[\hat b_{W}(A, O^{-})R\pi(A\mid O)]  ,\quad  \hat J_{\VM}= \E_{\tilde O\sim \nu_{\Ocal}}[\sum_a \hat b_V(a,\tilde O)],
\end{align*}
where $\E_{\Dcal}$ denotes the empirical average over all observed data. For instance, it is tuples $\mathcal{D}=\{(O_{i,t-1},O_{i,t},A_{i,t},R_{i,t},O_{i,t+1})\}_{i,t}$ where $i$ indexes the $i$th trajectory and $t$ indexes the $t$th time point.

%We also introduce the approach combining these two:
In addition, we can combine the aforementioned two estimators for policy evaluation. This yields the following doubly-robust estimator, $\hat J_{\DR}=\E_{\Dcal}[J(\hat b_W,\hat b_V)]$ where
\begin{align}\label{eqn:Jfg}
    J(f,g) \coloneqq \E_{\tilde O\sim \nu_{\Ocal}}[\sum_a g(a,\tilde O)]+ \frac{f(A,O^{-})}{1-\gamma}\{\{R+\gamma \sum_{a'}g(a',O^{+})\}\epol(A\mid O)-g(A,O)\}, 
\end{align}
for $f:\Acal\times \Ocal \to \RR$ and $g:\Acal\times \Ocal \to \RR$. 
%This approach has a doubly robust property as follows. %To see this, we show the following lemma. 
It has the desired doubly-robustness property, as shown in Section \ref{sec:theoryDRmethod}. %the following theorem. 
%This theorem immediately implies that 
%In other words,   

In fully observable MDPs, $\hat J_{\IS}$ reduces to the marginal IS estimator \cite{Liu2018}, and $\hat J_{\DR}$ reduces to the doubly-robust estimator \citep{KallusNathan2019EBtC}. %\cite{KallusNathan2019EBtC} \footnote{Recall $b_W$ corresponds to $d_{\epol}(s)/\bpol(a\mid s)$ and $b_V$ corresponds to $Q^{\epol}(a,s)/\epol(a\mid s)$ where $Q^{\epol}$ is a Q-function w.r.t $\epol$.  }. 
We remark that our proposal is not a trivial extension of these existing methods to the POMDP setting. The major challenge lies in developing identification formulas in \pref{thm:key_rl} to correctly identify the target policy's value. These results are not needed in settings without unmeasured confounders.
%Though the forms look similar to our proposed methods, it requires novel ideas to derive the proposed estimators beyond them. Our proposed estimators are based on the new identification theorem, \pref{thm:key_rl}. In contrast to the standard MDP setting, this identification part is highly nontrivial. 


Next, we present our proposal to estimate $b_V$ and $b_W$. To estimate $b_V$, a key observation is that, it satisfies the following integral equation,
\begin{align*}
   \forall f:\Acal\times \Ocal \to \RR, \quad \E[L_{\mathbb{V}}(b_V,f)]=0 
\end{align*}
where
\begin{align*}
    L_{\mathbb{V}}(g,f)=\{R \epol(A\mid O)+  \gamma \sum_{a'}g(a',O^{+})\epol(A \mid O)- g(A,O)\}f(A,O^-).
\end{align*}
%Being inspired by the general minimax estimation in \pref{sec:related}, 
This motivates us to develop the following minimax learning methods. Specifically, we begin with two function classes $\Vcal,\Vcal^{\dagger}\subset \{\Acal\times \Ocal \to \RR \}$ and  a regularization parameter $\lambda\in \mathbb{R}^+$. We next define the following minimax estimator,
\begin{align}\label{eqn:hatbV}
     \hat b_V=\argmin_{g\in \Vcal }\max_{f\in \Vcal^{\dagger}}\E_{\Dcal}[L_{\mathbb{V}}(g,f)]-\lambda \E_{\Dcal}[f^2]. 
\end{align}
Here, we use the function class $\Vcal$ to model the oracle value bridge function, and the function class $\Vcal^{\dagger}$ to measure the discrepancy between a given $g\in \Vcal$ and %is far from the genuine observed reward 
the oracle learnable value bridge function. In practice, we can use linear basis functions, neural networks, random forests, reproducing kernel Hilbert spaces (RKHSs), etc., to parameterize these functions. 
%Function classes $\Vcal,\Vcal^{\dagger}$ can be any function classes such as neural networks, random forests, and RKHSs. 
%The choice of $\lambda>0$ is arbitrary. Note 
In the fully observable MDP setting, the above optimization reduces to Modified Bellman Residual Minimization (MBRM) when $\lambda=0.5$ \cite{antos2008learning} and Minimax Q-learning (MQL) when $\lambda=0$ \cite{uehara2020minimax}. It is worthwhile to mention that fitted Q-iteration \citep[FQI,][]{ernst2005tree}, a popular policy learning method in MDPs, cannot be straightforwardly extended to the POMDP setting. This is because the regression estimator in each iteration of FQI will be biased under the POMDP setting.

%This is because even if $\gamma=0$, the naive regression is biased. 

Similarly, %to model the weight bridge function, 
according to \pref{eq:observed_reward}, %we introducing two function classes $\Wcal,\Wcal^{\dagger}\subset \{\Acal\times \Ocal \to \RR \}$ and $0<\lambda\in \mathbb{R}$; then, we define the following estimator:
we consider the following estimator for the weight bridge function, 
\begin{align}\label{eqn:hatbW}
     \hat b_W=\argmin_{g\in \Wcal }\max_{f\in \Wcal^{\dagger}}\E_{\Dcal}[L_{\mathbb{W}}(g,f)]-\lambda \E_{\Dcal}[f^2],
\end{align}
for some function classes $\Wcal,\Wcal^{\dagger}\subset \{\Acal\times \Ocal \to \RR \}$ and some $\lambda\in \mathbb{R}^+$.


%In particular, the estimators take simple forms in special cases such as when using linear models and RKHSs.  
%We remark that 
To simplify the calculation, we can use linear basis functions or RKHSs to parametrize these function classes. Specifically, when $\Vcal^{\dagger}$ or $\Wcal^{\dagger}$ is set to be the unit ball in an RKHS, then there exists a close form expression for the inner maximization problem \citep[see e.g.,][]{Liu2018}. When linear basis functions are used, the proposed minimax optimization has explicit solutions, as we elaborate below.
\begin{example}[Linear models]
Let $\Vcal=\Vcal^{\dagger}=\{(a,o)\mapsto \theta^{\top}\phi(a,o):\theta \in \Theta\}$ and $\lambda=0$, where $\phi:\Acal\times \Ocal \to \RR^{d}$ is a feature vector and $\Theta\subset \RR^d$. When the parameter space $\Theta$ is sufficiently large, it is immediate to see that
\begin{align*}
    \hat b_V = \prns{\E_{\Dcal}[\phi(A,O^{-})\phi^{\top}(A,O)] -\gamma  \E_{\Dcal}\bracks{\sum_{a'}\epol(A\mid O)\phi(A,O^{-})\phi^{\top}(a',O^+)} }^{+}\E_{\Dcal}[R \epol(A\mid O)\phi(A,O^-)]. 
\end{align*}
The resulting policy value estimator is given by
\begin{align*}
     \E_{\Dcal}[\sum_a\phi(a,O)]^{\top}\prns{\E_{\Dcal}[\phi(A,O^{-})\phi^{\top}(A,O)] -\gamma  \E_{\Dcal}\bracks{\sum_{a'}\epol(A\mid O)\phi(A,O^{-})\phi^{\top}(a',O^+)} }^{+}\E_{\Dcal}[R \epol(A\mid O)\phi(A,O^-)]. 
\end{align*}

Consider the standard MDP setting where $S=O=O^-,S^+=O^+$. By setting  $\Vcal=\{(s,a) \mapsto \theta^{\top}\epol(a\mid s)\phi(a,s)\},\Vcal^{\dagger}=\{(s,a) \mapsto \theta^{\top}\phi(a,s)/\epol(a\mid s)\}$, the above estimator reduces to classical LSTDQ estimator \cite{lagoudakis2003least}: 
\begin{align*}
     \E_{\Dcal}[\phi(\epol,S)]^{\top}\prns{\E_{\Dcal}[\phi(A,S)\phi^{\top}(A,S)] -\gamma  \E_{\Dcal}\bracks{\phi(A,S)\phi^{\top}(\epol,S^+)} }^{+}\E_{\Dcal}[R \phi(A,S)], 
\end{align*}
where $\phi(\epol,s)=\E_{a\sim \epol(s)}[\phi(a,s)]$. 
\end{example}








\subsection{Theoretical Results for Minimax Estimators} \label{subsec:theory}

We first investigate the nonasymptotic properties of the value function-based estimator $\hat J_{\VM}$ and the importance sampling estimator $\hat J_{\IS}$. We next study the asymptotic property of the DR estimator $\hat J_{\DR}$. Our results extend some recently established OPE theories in MDPs \citep{munos2008finite,chen2019information,KallusNathan2019EBtC,uehara2021finite} to the POMDP setting. We assume the observed dataset $\mathcal{D}$ consist of $n$ i.i.d. copies of $(O^-, O, A, R, O^+)$. This i.i.d. assumption is commonly employed in the RL literature to simplify the proof \citep[see e.g.,][]{dai2020coindice}.

%We next discuss the finite sample and asymptotic properties of IS and DR estimators ($\hat J_{\IS},\hat J_{\DR}$). 

\subsubsection{Value function-based and IS methods}\label{subsec:theory_value}

%We first establish the convergence rate of the estimated value bridge function. 
%show $\hat b_V$ converges to $b_V$. We first consider the 
We begin with the value function-based estimator. %in this section. 
First, to measure the discrepancy between the estimated learnable value bridge function $\hat b_V$ and $b_V$, %quantify the notion of convergence, 
we introduce the Bellman residual error for POMDPs as follows: 
\begin{definition}
The Bellman residual operator $\Tcal$% and Bellman operator $\Bcal$
%for a POMDP 
maps a given function $f: \Acal\times \Ocal\to \RR$ to another function $\Tcal f: \Acal\times \Ocal\to \RR$ such that
\begin{align*}
 %\{\Acal\times \Ocal\to \RR\} &\ni   f\mapsto 
 \Tcal f(a,o)=\E[R\epol(A\mid O)+\gamma  \sum_{a'}f(a',O^+)\epol(A\mid O)-f(A,O)\mid A=a,O^-=o],\quad \forall a,o.%\in \{\Acal\times \Ocal\to \RR\}. 
 % \{\Acal\times \Ocal\to \RR\}&\ni   f\mapsto \E[R\epol(A\mid O)+\gamma \E[\sum_{a'}f(a',O^+)\epol(A\mid O)\mid A,O^-]\in \{\Acal\times \Ocal\to \RR\}. 
\end{align*}
%Given a function $f:\Ocal\times \Acal\to \RR$, 
The corresponding bellman residual error is defined as $\E[\{\Tcal f(A,O^{-})\}^2]$.  
\end{definition}

%When $f$ is any observed reward bridge function $b_V$, the Bellman residual error is $0$. 
By definition, the Bellman residual error is zero for any learnable bridge function. As such, it 
%Thus, the Bellman residual error 
quantifies how a given function $f$ deviates from the oracle value bridge functions. In the MDP setting, it reduces to the standard Bellman residual error.  


%Now, we are ready to state the convergence result. 
We next establish the rate of convergence of $\hat b_V$ in the following theorem. 
\begin{theorem}[Convergence rate of minimax value bridge function estimators]\label{thm:con_results}
Set $\lambda$ in \eqref{eqn:hatbV} to $0.5$. Suppose (a) there exist certain learnable bridge function that satisfies \eqref{eqn:observed_value}; %. Suppose (a) 
(b) $\Vcal$ and $\Vcal^{\dagger}$ are finite hypothesis classes; (c) $\Vcal$ contains at least one learnable bridge function; (d) $\Tcal \Vcal\subset \Vcal^{\dagger}$; (e) There exist some constants $C_{\Vcal}$ and $C_{\Vcal^{\dagger}}$ such that $\forall v\in \Vcal,\|v\|_{\infty}\leq C_{\Vcal}$ and $\forall v\in \Vcal^{\dagger},\|v\|_{\infty}\leq C_{\Vcal^{\dagger}}$ Then, for any $\delta>0$, with probability $1-\delta$, 
\begin{align*}
    \E[\{\Tcal \hat b_V(A,O^{-})\}^2]^{1/2}\leq c \max(1,C_{\Vcal},C_{\Vcal^{\dagger}})\sqrt{\log(|\Vcal||\Vcal^{\dagger}|c/\delta)/n} 
\end{align*}
for some universal constant $c>0$. 
\end{theorem}

%Importantly, at this point,  
It is important to note that we only assume the existence of the learnable value bridge function in (a), \emph{not} the value bridge functions. This assumption is weaker since the class of learnable bridge functions is a larger function class and contains all bridge functions. 
%Recall the existence of observed bridge functions is weaker than the one of bridge functions. 
Assumption (b) can be further relaxed by assuming that $\Vcal$ and $\Vcal^{\dagger}$ are general hypothesis classes. In that case, the convergence rate will be characterized by the critical radii of function classes constructed by $\Vcal$ and $\Vcal^{\dagger}$. %For instance, when $\Vcal$ and $\Vcal^{\dagger}$ are $d$-dimensional models, $\log(|\Vcal||\Vcal^{\dagger}|)$ is $d$.
See e.g., \cite{uehara2021finite} for details.
Assumption (c) is the realizability assumption. Since learnable bridge functions are not unique, we only require $\Vcal$ to contain one of them. %is included in $\Vcal$. 
Assumption (d) is the (Bellman) completeness assumption. It requires that the discriminator class $\Vcal^\dagger$ is sufficiently rich and the operator $\Bcal$ is sufficiently smooth.  %\masa{how about now?}{\color{blue}wiggly. \{CS: can we use a different word?\}} 
In addition, we set $\lambda=0.5$ in Theorem \ref{thm:con_results} to simplify the proof. Similar results hold for any positive value of $\lambda$. 

These assumptions are valid in several examples. We elaborate below.
%are validated in several standard models. \masa{I add}
%The assumption (a) is also for simplicity. For general hypothesis classes, the rates are characterized by the critical radii of function classes constructed by $\Vcal$ and $\Vcal^{\dagger}$ like \cite{uehara2021finite}. For example, when $\Vcal$ and $\Vcal^{\dagger}$ are $d$-dimensional models, $\log(|\Vcal||\Vcal^{\dagger}|)$ is $d$. Especially, in the tabular setting, $\log(|\Vcal||\Vcal^{\dagger}|)$ is $|\Acal||\Ocal|$. 
\begin{example}[Tabular models]
Consider the tabular case, and $\Vcal$ and $\Vcal^{\dagger}$ are fully expressive classes, i.e., linear in the one-hot encoding vector over $(\Acal \times \Ocal)$.  Then, $\log(|\Vcal||\Vcal^{\dagger}|)$ is substituted by $|\Ocal||\Acal|$. The Bellman completeness $\Tcal \Vcal\subset \Vcal^{\dagger}$ is satisfied.  Our finite sample result circumvents the potentially complicated matrix concentration argument in POMDPs such as \citep{hsu2012spectral} by viewing the problem from the general perspective. 
\end{example}

\begin{example}[Linear models]
Consider the case where $\Vcal$ and $\Vcal^{\dagger}$ are linear models. Then, $\log(|\Vcal||\Vcal|^{\dagger})$ can be substituted by the dimension of the feature vector $d$. The Bellman completeness assumption is satisfied when $P_{\bpol}(R,O,O^+ \mid A,O^-)$ is linear in $\phi(A,O^-)$. In fully-observable MDPs, this reduces to the linear MDP model \citep{jin2020provably}, i.e.,  $P_{\bpol}(R,S^+ \mid A,S)$ is linear in $\phi(A,S)$. 
\end{example}


Next, we derive the convergence guarantee of the policy value estimator.  

\begin{theorem}[Convergence rate of value function-based estimators]\label{thm:final_policy}
Suppose the weight bridge functions $b'_W(\cdot)$ and learnable value bridge functions exist, and Assumption (a)-(e) in \pref{thm:con_results} hold.%\masa{i update here}
%the assumptions  hold. 
Then, for any $\delta>0$, with probability $1-\delta$, 
\begin{align*}
   | J(\epol)-\hat J_{\mathrm{VM}}| \leq c (1-\gamma)^{-1}\{\max(1,C_{\Vcal},C_{\Vcal^{\dagger}})\E[b'^2_W(A,O^{-})]\}^{1/2}\sqrt{\log(|\Vcal||\Vcal^{\dagger}|c/\delta)/n}.
\end{align*}
for some universal constant $c>0$. %is some universal constant. 
\end{theorem}
%Again, recall the existence of bridge functions ensures the existence of observed bridge functions. Elaborating on \pref{thm:con_results}, \pref{thm:final_policy} is easily proved by the following key equation:
Theorem \ref{thm:final_policy} requires a stronger condition than Theorem \ref{thm:con_results}, as we assume the existence of weight bridge function. %This corresponds to  \pref{thm:key_rl}. \masa{i update here}.
Its proof relies on the following key equation,
\begin{align*}
    |J(\epol)-\hat J_{\mathrm{VM}}|\leq \E[b'^2_W(A,O^{-})]^{1/2}\E[\{\Tcal \hat b_V(A,O^{-})\}^2]^{1/2},
\end{align*}
where the upper bound for the second term on the right-hand-side is given in Theorem \ref{thm:con_results}. 

Notice that Theorem \ref{thm:con_results} relies on the completeness assumption, e.g., Assumption (d). While this condition is necessary to obtain the nonasymptotic convergence rate of $\hat b_V,\hat b_W$, it is \emph{not} necessary to derive the convergence rate of the final policy value estimator. In the following, we show that when $b_V \in \Vcal,b_W \in \Vcal^{\dagger}$ %or $b_W \in \Wcal,b_V \in \Wcal^{\dagger}$, convergence rates of $\hat J_{\mathrm{IS}}$ or  $\hat J_{\VM}$ 
similar results can be established \emph{without} any completeness conditions. 

\begin{theorem}[Convergence rate without completeness]\label{thm:without}
Set $\lambda$ in equations \ref{eqn:hatbV} and \ref{eqn:hatbW} to zero.
Suppose (a) Assumption \ref{assum:existence} holds so that the bridge functions exist; (b) $\Vcal$ and $\Vcal^{\dagger}$ are symmetric finite hypothesis classes; (c) $\Vcal$ contains certain learnable reward bridge function; (d) $\Vcal^{\dagger}$ contains learnable weight bridge function; (e) $\forall v\in \Vcal,\|v\|_{\infty}\leq C_{\Vcal}$ and $\forall v\in \Vcal^{\dagger},\|v\|_{\infty}\leq C_{\Vcal^{\dagger}}$. Then, with probability $1-\delta$, 
\begin{align*}
  %\max( |J(\epol)-\hat J_{\mathrm{\VM}}|, |J(\epol)-\hat J_{\mathrm{IS}}|)
  |J(\epol)-\hat J_{\mathrm{VM}}| \leq   c \max(1,C_{\Vcal},C_{\Vcal^{\dagger}})^2(1-\gamma)^{-2}\sqrt{\log(|\Vcal||\Vcal^{\dagger}|c/\delta)/n},
\end{align*}
for some universal constant $c>0$. 
%where $c$ is some universal constant. 
\end{theorem}

%\subsubsection{IS methods}% and DR methods}
%We focus on the IS estimator in this section. 
Finally, we consider the IS estimator. To establish its convergence rate, we can define the adjoint Bellman residual operator $\Tcal'$ as in \cite{uehara2021finite}, and derive the convergence rate of $\E[\{\Tcal'\hat b_W(A,O^{+})\}^2]^{1/2}$ under realizability ($b_W\in \Wcal$) and (adjoint) completeness ($\Tcal' \Wcal\subset \Wcal^{\dagger}$). Similar to the proof of \pref{thm:final_policy}, this (adjoint) Bellman residual error can be translated into the error of the estimated policy value. Without the completeness assumption, similar results can be derived when $b_W \in \Wcal$ and $b_V \in \Wcal^{\dagger}$. 

%Notice that the completeness assumption is imposed in the above derivation. While this condition is necessary to obtain the nonasymptotic convergence rate of $\hat b_V,\hat b_W$, it is \emph{not} necessary to derive the convergence rate of the final policy value estimator. In the following theorem, we show that when $b_V \in \Vcal,b_W \in \Vcal^{\dagger}$ or $b_W \in \Wcal,b_V \in \Wcal^{\dagger}$, convergence rates of $\hat J_{\mathrm{IS}}$ or  $\hat J_{\VM}$ can be established \emph{without} any completeness conditions. 

\begin{comment}
\begin{theorem}[Convergence rate without completeness]\label{thm:without}
Set $\lambda$ in equations \ref{eqn:hatbV} and \ref{eqn:hatbW} to zero.
Suppose (a) Assumption \ref{assum:existence} holds so that the bridge functions exist; (b) $\Vcal$ and $\Vcal^{\dagger}$ are symmetric finite hypothesis classes; (c) $\Vcal$ contains certain learnable reward bridge function; (d) $\Vcal^{\dagger}$ contains learnable weight bridge function; (e) $\forall v\in \Vcal,\|v\|_{\infty}\leq C_{\Vcal}$ and $\forall v\in \Vcal^{\dagger},\|v\|_{\infty}\leq C_{\Vcal^{\dagger}}$. Then, with probability $1-\delta$, 
\begin{align*}
  \max( |J(\epol)-\hat J_{\mathrm{\VM}}|, |J(\epol)-\hat J_{\mathrm{IS}}|)\leq   c \max(1,C_{\Vcal},C_{\Vcal^{\dagger}})^2\sqrt{\log(|\Vcal||\Vcal^{\dagger}|c/\delta)/n}. 
\end{align*}
where $c$ is some universal constant. 
\end{theorem}
\end{comment}
% to true observed bridge functions

\subsubsection{DR methods}\label{sec:theoryDRmethod}
We focus on the DR estimator in this section. We first establish its doubly-robustness property such as \cite{robins1995semiparametric}  in Theorem \ref{thm:dr_infinite}. It implies that as long as either $\hat b_W$ or $\hat b_V$ is consistent, the final estimator $\hat J_{\DR}$ is consistent.
\begin{theorem}[Doubly-robustness property]\label{thm:dr_infinite}
Suppose Assumption \ref{assum:existence} holds. %, i.e., the existence of bridge functions.
%For any $f:\Acal\times \Ocal \to \RR$, we have $J(\epol)=\E[J(b_W,f)]=\E[J(f,b_V)] $. 
Then $J(f,g)$ defined in \pref{eqn:Jfg} equals $J(\epol)$ as long as either $f=b_W$ or $g=b_V$. 
\end{theorem}
%Most of the standard finite sample results \cite{uehara2021finite} and asymptotic results \cite{KallusNathan2019EBtC} in MDPs can be extended to the POMDP setting. We briefly showcase these results.  

%\paragraph{Convergence of $\hat b_W$. }  Following \cite{uehara2021finite}, we can similarly define the adjoint version of a Bellman residual operator $\Tcal'$ and derive the convergence result of $\E[\{\Tcal'\hat b_W(A,O^{+})\}^2]^{1/2}$ under realizability $b_W\in \Wcal$ and (adjoint) completeness $\Tcal' \Wcal\subset \Wcal^{\dagger}$. Then, this (adjoint) Bellman residual error is translated into the error of the policy value as  \pref{thm:final_policy}.  



%\paragraph{Convergence guarantees without completeness} All the convergence results mentioned so far are derived by assuming closedness conditions. While these conditions are apparently necessary to obtain the finite sample convergence guarantees of $\hat b_V,\hat b_W$ to true observed bridge functions,  this is \emph{not} necessary for the convergence of the final policy value estimator. When we assume $b_V \in \Vcal,b_W \in \Vcal^{\dagger}$ or $b_W \in \Wcal,b_V \in \Wcal^{\dagger}$ , we can still ensure the convergence of $\hat J_{\mathrm{IS}}$ or  $\hat J_{\VM}$ \emph{without} any completeness conditions.  The analogous result is seen in the unconfounded setting \cite{kallus2021causal,uehara2020minimax}. 




%\paragraph{Efficiency of $\hat J_{\mathrm{DR}}$.} 
We next show that $\hat J_{\mathrm{DR}}$ is efficient in the sense that it is asymptotically normal with asymptotic variance equal to the Cram\'er-Rao Lower Bound, e.g., the lower bound of MSEs of all regular OPE estimators in a locally asymptotic minimax sense \cite{VaartA.W.vander1998As}. To simplify the proof, we focus on the tabular setting where $\Scal,\Ocal$ are discrete spaces. We establish the corresponding the Cram\'er-Rao Lower Bound in the following theorem. 

\begin{theorem}\label{thm:cramer}
Suppose $\rank(\Pr_{\bpol}(\bO \mid A=a, \bO^{-}))=|\Scal|=|\Ocal|$ . The 
Cramer-Rao lower bound is 
\begin{align*}
     V_{\mathrm{EIF}}=\E[\phi^2_{\mathrm{EIF}}],\quad \phi_{\mathrm{EIF}}\coloneqq   (1-\gamma)^{-1}b_{W}(A,O^{-})\{ R\pi(A\mid O)+ \gamma \pi(A\mid O)\sum_{a^+}b_{V}(a^{+}, O^{+}) - b_{V}(A,O)  \}. 
\end{align*}
\end{theorem}
We remark when $\rank(\Pr_{\bpol}(\bO \mid A=a, \bO^{-}))=|\Scal|=|\Ocal|$, the bridge functions are uniquely defined, and so are the learnable bridge functions. Without such a uniqueness assumption, the Cram\'er-Rao Lower Bound is not well-defined. 
%as 
%This uniqueness is imposed to take derivatives of the inverse matrices. When they are not unique, since we need to take derivatives of Moore-Penrose inverses, the formal argument is much more intricate. Besides, more fundamentally, if bridge functions are not unique; thus, the lower bound notion is vacuous. 

%When Bellman residual errors are converted into L2 errors for the \emph{offline data}, we can show the DR estimator is efficient, i.e, the first-order term is the Cram\'er-Rao lower bound, which will be showed in \pref{sec:cramer}. 

Finally, we establish the asymptotic property of the DR estimator. 
%Here, 
%To alleviate some technical discussion associated with Donsker conditions, 
To avoid imposing certain Donsker conditions \citep{VaartA.W.vander1998As}, 
we focus on a sample-split version of $\hat J_{\mathrm{DR}}$ as in \cite{ZhengWenjing2011CTME}. It splits all data trajectories in $\Dcal$ into two independent subsets $\Dcal_1,\Dcal_2$, computes the estimated bridge function $\hat b^{(1)}_V,\hat b^{(1)}_W$ ($\hat b^{(2)}_V,\hat b^{(2)}_W$) based on the data subset in $\Dcal_2$ ($\Dcal_1$), and does the estimation of the value based on the remaining dataset. Finally, we aggregate the
resulting two estimates to get full efficiency. This yields the following DR estimator, %parameter, i.e., the value %$\hat b^{(2)}_V,\hat b^{(2)}_W$ based on $\Dcal_1$.  this is defined by 
\begin{align*}
    \hat J^{*}_{\mathrm{DR}}=0.5 \E_{\Dcal_1}[ J(\hat b^{(1)}_W,\hat b^{(1)}_V)]+0.5 \E_{\Dcal_2}[ J(\hat b^{(2)}_W,\hat b^{(2)}_V)]. 
\end{align*}
We summarize the results in the following theorem.
\begin{theorem}\label{thm:efficiency}
Assume the existence and uniqueness of bridge and learnable bridge functions. Suppose $\hat b_W,b_W,\hat b_V,b_V$ are uniformly bounded by some constants, $\E[\{\hat b^{(j)}_W- b^{(j)}_W\}^2(A,O^{-})]=o_p(1),\E[\{\Tcal \hat b^{(j)}_V(A,O^{-})\}^2]=o_p(1), \\ \E[ \{\sum_a\hat b^{(j)}_V(a,O)-b^{(j)}_V(a,O) \}^2 ]^{1/2}=o_p(1),\E[\{\hat b^{(j)}_W- b^{(j)}_W\}^2(A,O^{-})]^{1/2}\E[\{\Tcal \hat b^{(j)}_V(A,O^{-})\}^2]^{1/2}=o_p(n^{-1/2})$ for $j=1,2$. Then, $\sqrt{n}(\hat J^{*}_{\DR}-J(\epol))$ weakly converges to a normal distribution with mean 0 and variance $V_{\mathrm{EIF}}$. 
\end{theorem} 

We again, make a few remarks. First, although the estimated bridge functions are required to satisfy certain nonparametric rates only, the resulting value estimator achieves a parametric rate of convergence (e.g. $n^{-1/2}$). This is essentially due to the doubly-robustness property, which ensure that the bias of the estimator can be represented as a product of the
difference between the two estimated bridge functions and their oracle values. In comparison, \pref{thm:final_policy} requires the estimated bridge function to satisfy the parametric convergence rate. This is an advantage of the DR estimator over the value function-based estimator. 

%While the conditions here permit the nonparametric rates for nuisance estimators, the final rate of $\hat J^{*}_{\DR}$  is parametric. Comparing to \pref{thm:final_policy}, which requires parametric rates for nuisance estimators to obtain the parametric rate for the policy value, the implied result here is stronger. 


Second, \pref{thm:efficiency} derives the asymptotic variance of $\hat J^{*}_{\DR}$, which can be consistently estimated from the data. %This allows us to quantify the uncertainty of the DR estimator. T
This allows us to perform a handy Wald-type hypothesiss testing.  
%his allows us to 
%\masa{add}

%Though this theorem is appealing to perform statistical inference, it 
Finally, \pref{thm:efficiency}
requires a stronger assumption, i.e., the uniqueness of bridge functions, which implies that $|\Scal|=|\Ocal|$. Without this assumption, it remains unclear how to define the $L_2$ error of the estimated bridge function.  %\masa{ $L^2$?} 
%This is due to the fact that L2 errors become vacuous if bridge functions are not unique. How to relax this assumption is our future work. 
%While the finite sample guarantees of $\|\hat b_W-b_W\|^2_2,\|\hat b_V-b_V\|^2_2$ , 




%When the spaces are continuous or $|\Scal|\neq |\Ocal|$, the formal argument is much more subtle. Irrespective of that, this result is still useful to comp up with DR estimators. 

%\subsection{Cram\'er-Rao Lower Bound }\label{sec:cramer}

%Efficiency bounds are defined for the target functional and the posited models. 
%When the models are parametric, they are known as Cramer-rao lower bounds. Efficiency bounds are the natural extension of Cramer-Rao lower bounds from parametric to nonparametric models. Roughly, this gives the lower bound of MSE in a locally asymptotic minimax sense.  Estimators asymptotically achieve these bounds are called efficient estimators. All efficient estimators are equal to $\EE[\phi_{EIF}]+o_p(n^{-1/2})$. 

%When $\Scal,\Ocal$ are finite spaces, we can derive the Cram\'er-Rao lower bound of the policy value $J(\epol)$. This provides the lower bound of MSEs in a locally asymptotic minimax sense \cite{VaartA.W.vander1998As}.


